T*$\varepsilon$ -- Bounded-Suboptimal Efficient Motion Planning for Minimum-Time Planar Curvature-Constrained Systems

We consider the problem of finding collision-free paths for curvature-constrained systems in the presence of obstacles while minimizing execution time. Specifically, we focus on the setting where a planar system can travel at some range of speeds with unbounded acceleration. This setting can model many systems, such as fixed-wing drones. Unfortunately, planning for such systems might require evaluating many (local) time-optimal transitions connecting two close-by configurations, which is computationally expensive. Existing methods either pre-compute all such transitions in a preprocessing stage or use heuristics to speed up the search, thus foregoing any guarantees on solution quality. Our key insight is that computing all the time-optimal transitions is both~(i)~computationally expensive and~(ii)~unnecessary for many problem instances. We show that by finding bounded-suboptimal solutions (solutions whose cost is bounded by $1+\varepsilon$ times the cost of the optimal solution for any user-provided $\varepsilon$) and not time-optimal solutions, one can dramatically reduce the number of time-optimal transitions used. We demonstrate using empirical evaluation that our planning framework can reduce the runtime by several orders of magnitude compared to the state-of-the-art while still providing guarantees on the quality of the solution.

==> Makefile <==
PDFLATEX := pdflatex
BIBTEX   := bibtex

TARGET   := main

pdf: 
	$(PDFLATEX) $(TARGET).tex
#	latex $(TARGET).tex
#	dvips $(TARGET).dvi -o $(TARGET).ps -t letter -Ppdf -G0
#	ps2pdf $(TARGET).ps 


all: pdf pic
	$(MAKE) -C . bib
	$(MAKE) -C . pdf
	@echo -e "\033[0;33m"
	$(MAKE) -C . pdf
	@echo -e "\033[0m"
#	xdg-open $(TARGET).pdf


bib:
	@echo -e "\033[0;32m"
	$(BIBTEX) $(TARGET)
	@echo -e "\033[0m"

pic:
	mkdir -p fig
	$(MAKE) -C support copy

plots: 
#	cd experiments/scripts ; R -f plot-all.R ; cd -
#	cp experiments/scripts/plots/*.pdf support/pdf

open o: all
	xdg-open $(TARGET).pdf

clean c:
	$(RM) -rv $(TARGET).log $(TARGET).aux $(TARGET).toc $(TARGET).lof $(TARGET).lot $(TARGET).loa $(TARGET).blg $(TARGET).ps $(TARGET).out $(TARGET).dvi $(TARGET).bbl
	$(RM) -rv $(TARGET).synctex.gz

cleanall ca: clean
	$(RM) -rv $(TARGET).pdf $(TARGET).bbl
	$(RM) -rf fig/.done
	
x:
	make ca
	make plots
	make pic
	make



==> src/remove.tex <==
% Filename: remove.tex
% Date:     2021/09/08 18:02
% Author:   Jan Faigl

% - main.tex ------------------------------------------------------------------
% \documentclass{article}
\usepackage{subcaption}
\usepackage[style=ieee]{biblatex}

%\renewcommand{\vec}[1]{\overrightarrow{#1}}
%\tstareps- sub-optimal minimum-time Motion-Planning Algorithm For Curvature-Constrained Systems
% Near-Optimal Motion-Planning Algorithm For Fast Solution In Curvature-Constrained Systems

% \textbf{{\textit{Abstract}}---A sub-optimal minimum-time motion-planning algorithm, called~\tstareps, is presented in this paper for curvature-constrained variable-speed robotic-systems. 
% It finds a collision-free solution more quickly than the optimal solution that is found by~\tstar algorithm, especially if environmental conditions change when offline prepossessing can not take place. 
% Our algorithm allows us to balance the quality of the solution and the runtime. 
% The cost of the solution that is found by~\tstareps is constrained by the conjecture factor \eps. The solution cost is at most \eps times the optimal cost. 
% The runtime improvement is achieved by reducing the most computationally expensive portions of the optimal algorithm, optimizations for obtaining an approximation to time-optimal transitions between the robotic-system configurations. 
% Using instances with wind, we demonstrate the effectiveness of the algorithm.~\tstareps is used here to deal with a motion-planning problem in a grid-based space. 
% Furthermore, the approach can be generalized and also used in continuous space to reduce the number of edge evaluations which is the most computationally expensive in continuous space.}

% \textbf{{\textit{Abstract}} --- 
% % Minimum-time motion-planning algorithms for curvature-constrained robotic-systems aim to find a path with the lowest execution time. 
% % They have applications in domains such as medical robots, agriculture, and autonomous cars. 
% % Finding the collision-free optimal path in the presence of obstacles can be challenging, no algorithm solves the problem in polynomial time. 
% % % In addition, the approximate solution involves computational demanding time-optimal transitions optimization process.
% % The time-optimal algorithm, called~\tstar, solves this problem in grid-based space. However, it demands high computationally effort.
% % % In addition, the time-optimal algorithm, called~\tstar, demands high computationally effort.
% % % We extended~\tstar approach and propose a novel sub-optimal algorithm, called \boldtstareps, that reduces the number of optimizations during the search after a solution.~\boldtstareps incrementally computes time-optimal transitions only for those who have a high probability to be part of a bounded-suboptimal solution.
% % We extended~\tstar approach and propose a novel bounded-suboptimal algorithm, called~\boldtstareps, that reduces computationally effort and hence the runtime.
% % The cost of the solution that is found by~\boldtstareps is bounded by the approximation factor of~$\boldsymbol{1+\varepsilon}$ of an optimal path.
% % We demonstrate~\boldtstareps's efficacy in dynamic environmental conditions and it shows significant computational time reduction compare to the state-of-the-art optimal algorithm.
% \DP{
% %  What is the problem?
% Motion-planning algorithms for minimum-time curvature-constrained systems aim to find a path with the lowest execution time.
% % Why is it relevant?
% Those algorithms have applications in domains such as medical robots, agriculture, and autonomous vehicles. 
% % Why is it hard?
% % NP-hard to decide if the curvature-constrained path is collision-free.
% Determining if a path of a curvature-constrained system is collision-free can be challenging, no algorithm solves this problem in polynomial time.
% % What have others done?
% % Found an optimal path in discrete space.
% The algorithm, called~\tstar, finds a time-optimal collision-free path in a grid-based space with the presence of obstacles for a variable-speed system.
% % What's missing?
% % Requires expensive-to-compute and unnecessary transitions between the system configurations.
% Unfortunately, it demands many expansive and often unnecessary computations of transitions between the system configurations.
% % What is our ONE key insight?
% % Reuse of already computed transitions.
% We propose a novel, bounded-suboptimal motion-planning algorithm for minimum-time curvature-constrained systems, called~\boldtstareps.
% The algorithm reduces the computational effort by reuse of already expensive-to-compute transitions.
% It finds a path of a bounded cost with an approximation factor of~$\boldsymbol{1+\varepsilon}$ of an optimal path.
% % How do we compare against the state of the art?
% % Order of magnitude faster, especially in dynamic.
% We demonstrate the efficacy of~\boldtstareps compare to the state-of-the-art approach and that it can reduce the runtime by an order of magnitude, especially in dynamic environmental conditions.
% }
% }

% \textbf{\textit{Abstract} --- 
% \DP{
% Minimum-time curvature-constrained motion planning algorithms seek the path with the smallest execution time.
% % Why is it relevant?
% Medical robots, agriculture, and autonomous vehicles all use these algorithms. 
% % Why is it hard?
% % NP-hard to decide if the curvature-constrained path is collision-free.
% The problem of determining if a path of a curvature-constrained system is collision-free can be challenging. No algorithm can solve this problem in polynomial time.
% % What have others done?
% % Found an optimal path in discrete space.
% The algorithm, called~\tstar, finds a time-optimal collision-free path for such a system with variable-speed in a grid-based space.
% % What's missing?
% % Requires expensive-to-compute and unnecessary transitions between the system configurations.
% Nevertheless, many expensive and often unnecessary computations are required for the transition between system configurations.
% % What is our ONE key insight?
% % Reuse of already computed transitions.
% A new, bounded-suboptimal motion-planning method for minimum-time curvature-constrained systems called~\boldtstareps is presented.
% As a result of reusing expensive-to-compute transitions, the algorithm helps reduce computational effort.
% Finding a path of a bounded cost with an approximation factor of~$\boldsymbol{1+\varepsilon}$ of an optimal path is resolved through this algorithm.
% % How do we compare against the state of the art?
% % Order of magnitude faster, especially in dynamic.
% The efficiency of \boldtstareps can reduce runtime by an order of magnitude compared to the state-of-the-art approach and is particularly effective in dynamic environmental conditions.
% }
% }

\printbibliography

% - abstract.tex --------------------------------------------------------------
\ignore{
\textbf{\textit{Abstract} --- 
\DP{
\emph{Curvature-constrained} motion planning is a fundamental capability in various systems, including medical robots, agricultural machines, and urban vehicles. In many practical settings,  it is also desirable to produce \emph{minimum-time} plans, which minimize time to execution, to increase throughput and reduce operational cost, while also satisfying collision avoidance and curvature-constraints. 
All of those requirements give rise to a complex problem setting for which existing approaches tend to require prohibitively large running times. This limits the applicability of curvature-constrained systems in practice. 
We present~\boldtstareps, a bounded-suboptimal motion-planning algorithm for minimum-time curvature-constrained systems. 
Our algorithm reduces the computational burden of \tstar (Song et al., 2018)---a state-of-the-art grid-based planner for curvature-constrained systems---by a clever reuse of expensive-to-compute transitions, and finds a bounded cost path with an approximation factor of~$\boldsymbol{1+\varepsilon}$ of the optimum execution time. 
We test the efficacy of~\boldtstareps on various scenarios and demonstrate that it can significantly reduce runtime while achieving a high-quality solution, when compared to~\tstar, especially under dynamic environmental conditions. 
}
}
}


% - intro.tex -----------------------------------------------------------------
% What is the problem?
%\DP{Motion-planning algorithms for curvature-constrained robotic-system, systems with a minimum turning radius which they must follow, are designed to find a path from given start to end configurations of the system.}
% Why is it relevant?
% Curvature constrains are prevalent in a variety of systems including steerable needles~\cite{needle}, 
% autonomous aerial vehicles~\cite{autonomous_Ariel}, 
% autonomous cars~\cite{autonomous_Car} and autonomous underwater vehicles~\cite{garau2009path}.
%and the specific model we consider, a planar variable-speed curvature-constrained systems with no acceleration bounds. %\DP{when speed changes can be made instantly,} 
%This problem is directly applicable to planning paths for systems such as fixed-wing drones.
% Why is it hard?
% Unfortunately, collision-free curvature-constrained motion planning is NP-hard already for point robots operating in the plane~\cite{NP_hard}.
% What have others done?

% What's missing?
% What is our ONE key insight?
% How do we compare against the state of the art?

% What are our contributions?
% What are our limitations?

% \DP{We use this lower bound for both speedup the computational time and for ensure the solution quality.}

% \footnote{\DP{I think this paragraph is to technical to the intro section}}. 
%
%\footnote{There are some approaches that use local information regarding if an edge is collision free or not to inform the planner such introduced in~\cite{jimenez1998collision}\footnote{\OS{This talks about general CD,~we need a ref to show how information about one edge is used to reduce CD for another edge. Perhaps a learning-based approach.}} but these are beyond the scope of the discussion here}. 

%As we will see,~in certain dynamic conditions such as planning under wind currents,~these transitions cannot be pre-computed in advance.\footnote{\DP{Consider to remove. This is the first time both dynamic condition and pre-compute are mentioned. But without a context.}} 


% paper outline 
\ignore{
Many physical systems can be modeled as curvature constrained,~such as steerable needles~\cite{needle},~autonomous aerial vehicles~\cite{autonomous_Ariel},~autonomous cars~\cite{autonomous_Car} and autonomous agricultural robots~\cite{agriculture}. 
The specific model we consider is directly applicable to planning paths for systems such as fixed-wing drones.
Unfortunately,~even deciding if a collision-free curvature-constrained path exists between two given poses is NP-hard~\cite{NP_hard}.
% Motion-planning problems for curvature-constrained systems, systems with a minimum turning radius which they must follow, are investigated broadly. 
% Lazard et al.~\cite{NP_hard} showed that the problem of deciding whether a curvature-constrained collision-free path exists between two given poses in the presence of polygonal obstacles is NP-hard, which means that no polynomial-time exact algorithm exists for curvature-constrained motion-planning in arbitrary environments.

% In the context of static environment conditions, Dubins~\cite{Dubins} analyzed the shortest path connecting two points in the two-dimensional Euclidean plane~(i.e. x-y plane) for a curvature-constrained point robot. 
% He used a geometric approach and showed that the shortest path between a pair of curvature-constrained poses, also called configurations, must be one of six optional paths that include straight and curved segments. These six types of paths are known as Dubins paths. 
% Dubins paths assume that the system can turn at a constant radius, i.e. constant velocity. Dubins paths are commonly used because they provide an analytical, simple to calculate expression. 


% \begin{figure}[!t]
%     \centering
%     \begin{subfigure}{.24\textwidth}
%         \includesvg[width=1\linewidth]{pics/Map6_tstar_wo_wind.svg}
%         % {\includegraphics[scale=0.6]{pics/Lower bound quality}}
%         \caption{}
%     \end{subfigure}
%     \begin{subfigure}{.24\textwidth}
%         \includesvg[width=1\linewidth]{pics/tstar-eps_2_map6_no_wind.svg}
%         % {\includegraphics[scale=0.6]{pics/Lower bound quality}}
%         \caption{}
%     \end{subfigure}
%     \begin{subfigure}{.55\textwidth}
%         \vspace{2mm}
%         \includesvg[width=1\linewidth]{pics/tstar and tstar-eps_2_map6_transitions.svg}
%         % {\includegraphics[scale=0.6]{pics/Lower bound quality}}
%         \caption{}
%     \end{subfigure}
%     \caption{The time-optimal solution is obtained by~\tstar~(a) and bounded-suboptimal path found by~\tstareps where~$\varepsilon=1$~(b). The robotic-system can travel either at minimum~(red) or maximum~(green) speed. The path costs of~\tstar and~\tstareps are~35.06 and~35.45 sec, respectively. The runtime of~\tstar and~\tstareps are~35.86 sec and~1.99 sec, respectively. In the eight neighbors and eight optional heading angles setup, the number of transitions to calculate is reduced when symmetry and rotation are used. Any start position has either horizontal or diagonal. Notice that~\tstareps calculates significantly fewer transitions, whereas~\tstar calculates many transitions that it does not use in the found path~(c).}
%     \label{fig:transitions_compare}
% \end{figure}
\begin{figure}[!t]
    \centering
    \begin{subfigure}{.24\textwidth}
        \includesvg[width=1\linewidth]{pics/Map6_tstar_wo_wind.svg}
        % {\includegraphics[scale=0.6]{pics/Lower bound quality}}
        \caption{}
        \label{fig:transitions_compare-a}
    \end{subfigure}
    \begin{subfigure}{.24\textwidth}
        \includesvg[width=1\linewidth]{pics/tstar-eps_1_3_map6_no_wind.svg}
        % {\includegraphics[scale=0.6]{pics/Lower bound quality}}
        \caption{}
        \label{fig:transitions_compare-b}
    \end{subfigure}
    \begin{subfigure}{.5\textwidth}
        \vspace{2mm}
        \includesvg[width=1\linewidth]{pics/tstar and tstar-eps_1_3_map6_transitions_on_two_cells.svg}
        % {\includegraphics[scale=0.6]{pics/Lower bound quality}}
        \caption{}
        \label{fig:transitions_compare-c}
    \end{subfigure}
    \caption{
    \protect
    The time-optimal solution is obtained by~\tstar~\subref{fig:transitions_compare-a}(a) and bounded-suboptimal path found by~\tstareps where~$\varepsilon= 0.3$~(b). The robotic-system can travel either at minimum~(red) or maximum~(green) speed. 
    %
    The path costs of both~\tstar and~\tstareps is~$35.06$ sec. 
    The runtime of~\tstar and~\tstareps are~$35.86$ sec and~$2.76$ sec, respectively. 
    In the eight neighbors and eight optional angular headings setting, the number of transitions to calculate is reduced when symmetry and rotation are used. 
    Any start position has either horizontal or diagonal orientation. Notice that~\tstareps computes significantly fewer transitions, whereas~\tstar computes many transitions that it does not use in the found path~(c).}
    \label{fig:transitions_compare}
\end{figure}

% In this work we are interested in planning for curvature-constrained planar systems such as fixed-wing drones. We start by briefly reviewing different kinematic models and then continue to describe approaches used to plan for such models.

To this end, the continuous planning problem is typically discretized into a graph data structure using sampling-based~\cite{karaman2011sampling} or search based approaches~\cite{hart1968formal}. 
Here vertices correspond to robot configurations (i.e.,~$d$-dimensional points that uniquely describe the robot's position and orientation) and edges correspond to locally motions taken by the robot.
Dubins~\cite{Dubins} analyzed the shortest path connecting two points in the two-dimensional Euclidean plane~(i.e. x-y plane) for a curvature-constrained point robot. 
Wolek et al.~\cite{Wolek} derived an approximate solution to find the time-optimal path between two poses of a curvature-constrained variable-speed vehicle in an obstacle-free space.
Song et al.~\cite{T*} presented a time-optimal risk-aware motion-planning algorithm in the presence of obstacles for variable-speed system in discrete space. 
The optimal solution path of curvature-constrained system that able to travel at variable-speed, demands significant computation resources. 
Most of the computation effort directed to compute time-optimal path between pair of poses, called transitions.

This work aim to solve the problem of motion-planning for minimum-time curvature-constrained system more efficiently.
This comes from obtaining sub-optimal solution that aims to computes as few as possible time-optimal transitions by using lazy approach~\cite{lazy_search} and lower bounds for true cost of transitions for many of them.
Our algorithm, called~\tstareps, allows reducing planning times by orders of magnitude when compared to the state-of-the-art, especially in dynamic environmental conditions when the all time-optimal transitions can not be computed beforehand.

\DP{I think the figure notation fits more to the algorithmic background when the reader has better knowledge abound~\tstar. However, I'm afraid this is to far from the beginning of the paper.}

Fig.~\ref{fig:transitions_compare} demonstrates this insight.
The optimal solution, found by~\tstar, uses only a small fraction of the calculated time-optimal transitions.~\tstareps computes in this scenario only a small fraction of all transitions for its solution Fig.~\ref{fig:transitions_compare}~(c).
Therefore, the majority of the transitions do not have to be calculated. 
Since those calculations are the most computationally expensive part of the algorithm, reducing those calculations can save a significant amount of computational time.

Our contribution is that using the understanding that computing all the time-optimal transitions is both~(i)~computational expensive and~(ii)~unnecessary for many problem instances, bounded-suboptimal paths in the presence of obstacles can be efficiently computed.

The algorithm limitation is that in many cases, it computes more time-optimal transitions than it needs for its sub-optimal solution. 
When high solution quality is required, it can compute all possible.
\newpage

% Time-optimal motion-planning algorithms are designed to find the optimal solution to a problem where the objective is to minimize the duration of solution execution. This minimum-time path can be also called the time-optimal path. 


% When the system is constrained to travel at a single speed, an optimal path connecting two configurations~(i.e., two planar locations, each associated with its angular heading) can be computed analytically~\cite{Dubins}. 
% In this setting, an optimal path, also know as a~\emph{Dubins path} can be described by the system making a ``right turn~(R)'' , ``left turn~(L)'' or going ``straight~(S)'', and an optimal path will always be at least one of the six types: RSR, RSL, LSR, LSL, RLR, LRL. 
% Since the system travels at a single speed, in this model the shortest path and time-optimal path are identical.
% Time-optimal motion-planning algorithms are designed to find the optimal solution to a problem where the objective is to minimize the duration of solution execution. This minimum-time path can be also called the time-optimal path. 

% \begin{figure}[!t]
%     \centering
%     % \adjustbox{margin=1em,width=\textwidth,set height=4cm,set depth=4cm,frame,center}{\includegraphics[scale=0.6]{pics/Lower bound quality}}
%     \includesvg[scale=0.55]{pics/unique_transitions.svg}
%     % {\includegraphics[scale=0.6]{pics/Lower bound quality}}
%     \caption{The number of unique transitions in~\tstar solution vs. the number of configurations in the solution. The figure shows a comparison between several maps where each has a different portion of the map occupied by obstacles. The red line represents the maximum number of unique transitions that in static environmental conditions reduced using symmetry and rotation to~68.}
%     \label{fig:unique_transitions}
% \end{figure}

% The next kinematic model, which is the focus of this work, is the setting where the system can travel at some range of speeds but with unbounded acceleration~(i.e., transitioning between low and high-speed can be done instantaneously). 
% It is not hard to see that in this setting the shortest path is attained by computing the optimal Dubins path assuming that the system travels at minimum speed~(as the system can travel using larger turning radii and can thus better maneuver). 
% Computing the time-optimal path is more involved and requires alternating between low speed~(to allow for tighter turns) and high-speed motions~(to allow for faster progress).

% Kučerová et al.~\cite{kuvcerova2020finding} showed it is time-efficient to combine various turning radii. 
% Their approach finds a path with a cheaper time-cost than Dubins path.
% Wolek et al.~\cite{Wolek} showed that it is sufficient to consider only the two extreme speeds and identified a sufficient set of 34 candidate paths, where each candidate path contains circular arcs or straight-line segments on which the vehicle can travel at either of the two extreme speeds. 
% In contrast to Dubins path which can be computed analytically, computing the time-optimal paths for a variable-speed system requires a numerical optimization that is~(i) much more computational expensive and~(ii) may return locally optimal solutions~(and not globally-optimal).
% Song et al.~\cite{T*} presented a time-optimal risk-aware motion-planning algorithm in the presence of obstacles for variable-speed system. 
% This algorithm, called~\tstar, achieves the time-optimal solution but consumes a long-time offline optimization process. 
% Wilson et al.~\cite{GMDM} developed a fast, collision-free path finding algorithm that uses multi-speed Dubins path to reduce the computational effort and runtime. 
% % Their algorithm solution cost is not much more than the optimal for the settings demonstrated, but there are no guarantees of the quality, or how far from the optimal the solution cost will be.
% For the settings demonstrated, the algorithm solution cost is not much more than optimal, but no guarantees are made as to its quality, or how far from optimal it will be.

% Wolek et al.~\cite{Wolek} derived an approximate solution to find the time-optimal path for a curvature-constrained variable-speed vehicle in an obstacle-free space. 
% Under the assumption that the vehicle can travel at two extreme speeds. 
% They identified a sufficient set of~34 candidate paths, where each candidate path contains circular arcs or straight-line segments on which the vehicle can travel at either of the~two extreme speeds. %However, in their work, Wolek et al. did not consider the presence of obstacles. 
% Song et al.~\cite{T*} presented a time-optimal risk-aware motion-planning algorithm in the presence of obstacles in grid-based space. 
% This algorithm, called~\tstar, achieves the time-optimal solution but consumes a long-time offline optimization process. 
% Wilson et al.~\cite{GMDM} developed a fast, collision-free path finding algorithm that uses multi-speed Dubins path to reduce the computational effort and runtime. 
% % Their algorithm solution cost is not much more than the optimal for the settings demonstrated, but there are no guarantees of the quality, or how far from the optimal the solution cost will be.
% For the settings demonstrated, the algorithm solution cost is not much more than optimal, but no guarantees are made as to its quality, or how far from optimal it will be.

% Motion-planning under dynamic environment conditions of curvature-constrained systems is investigated~\cite{selecky2013wind},~\cite{garau2009path} because it is directly related to real-world problems and aims to deal with real-world conditions.
% % Wu et al.~\cite{multi-astar} proposed multi-objective cost functions to find the shortest path of an unmanned aerial vehicle~(UAV) in dynamic uncertain environments. Their algorithm, called multi-step~\astar~(\msastar), finds the optimal solution while taking into account several variables such as length, angle, and velocity trajectory segments. 
% % \msastar finds paths of equivalent cost but in much less computational time than~\astar algorithm.
% McGee et al.~\cite{optimal_trajectory_with_currents} studied the minimum-time path planning problem in constant wind for curvature-constrained vehicles. 
% They presented the optimal solution for the problem for free-space and constant velocity scenarios. 
% Mittal et al.~\cite{Dubins_with_currents} used only two types of Dubins paths to compute the path between two vehicle pose under ocean currents. 
% They do so because only those two have analytical expression.
% The remaining four require solving a root-finding problem that demands a long computational time. 
% The solution is reached faster than if all six were computed. 
% However, this method doesn't consider variable speed nor obstacles. 

% \DP{Not sure how this paragraph is incorporated the above}
% All the above works are similar in the sense that they focus on either the shortest or time-optimal path. 
% To our knowledge, there is no existing motion-planning algorithm that uses the shortest path solution for a given problem as a heuristic to minimize the time. 
% In addition, a bounded-suboptimal motion-planning algorithm for minimum-time curvature-constrained systems which bound the solution quality has not been developed.

% To this end, we introduce~\tstareps, a new bounded-suboptimal motion planning algorithm for a minimum-time curvature-constrained system in grid-based space.
% In grid-based search, there is a finite number of edge types in the search graph.
% Those edges are also called transitions between the graph's vertices.
% For the case of variable-speed systems, the evaluation of those time-optimal transitions is computationally expensive.

% Our key insight is that the shortest and time-optimal paths are related, as shown by the fact that they are typically in the same homotopy class, i.e there is a continuous deformation between them without going through obstacles. This relationship can reduce a significant amount of computation time, and using a bounded-suboptimal searching algorithm that has an upper bound on the quality of the solution, we can balance the path cost and the runtime. 
% Our key insight is derived from our experience that in most cases, grid-based solutions don't incorporate all the possible time-optimal transitions. 
% In particular, it only constitutes a small fraction of all possible transitions.
% Fig.~\ref{fig:transitions_compare} demonstrates this insight.
% The optimal solution, found by~\tstar, uses only a small fraction of the calculated time-optimal transitions.~\tstareps computes in this scenario only a small fraction of all transitions for its solution Fig.~\ref{fig:transitions_compare}~(c).
% Therefore, the majority of the transitions do not have to be calculated. 
% Since those calculations are the most computationally expensive part of the algorithm, reducing those calculations can save a significant amount of computational time.
% The main contributions and advantages of this work are as follows:
% \begin{enumerate}
%     \item We present a sub-optimal minimum-time motion-planning algorithm for curvature-constrained systems in the presence of obstacles, called~\tstareps, which allows finds paths faster than the optimal algorithm, especially in dynamic environmental conditions.
%     \item~\tstareps suggest a sub-optimal solution with an upper bound on the quality.
%     \item Reducing computational effort with a novel approach that uses both the shortest and time-optimal paths.
%     % \item There were several possible lower bounds for time-optimal transitions between successive configurations tested and an informative one identified.
% \end{enumerate}
% The main contribution and advantages of this work is that we present a sub-optimal motion-planning algorithm for minimum-time curvature-constrained systems in the presence of obstacles, called~\tstareps, which allows finds paths faster than the optimal algorithm, especially in dynamic environmental conditions.
% The main contribution and advantage of this work are that we present a bounded-suboptimal motion-planning algorithm for minimum-time curvature-constrained systems in the presence of obstacles, called~\tstareps.
% The algorithm allows finds paths without calculating all possible time-optimal transitions between consecutive configurations of the robotic-system. 
% This allows us to find a solution faster than the optimal algorithm, especially in dynamic environmental conditions.
% We demonstrate the effectiveness of the algorithm, concerning runtime, thanks to the reduction of time-optimal transition optimizations when compared to a state-of-the-art algorithm.
% The main contribution and advantage of this work are that we present a bounded-suboptimal motion-planning algorithm for minimum-time curvature-constrained systems in the presence of obstacles.
% The algorithm allows finds paths without calculating all possible time-optimal transitions between consecutive configurations of the system. 
% This allows us to find a solution faster than the optimal algorithm, especially in dynamic environmental conditions.
% We demonstrate the effectiveness of the algorithm, concerning runtime, thanks to the reduction of time-optimal transition optimizations when compared to a state-of-the-art algorithm.
}

% - related.tex ---------------------------------------------------------------

%In this setting, an optimal path, also know as a~\emph{Dubins path} can be described by the system making a ``right turn~(R)'', ``left turn~(L)'' or going ``straight~(S)'', and an optimal path will always be at least one of the six types: RSR, RSL, LSR, LSL, RLR, LRL.

% \footnote{\DP{Consider to move the description on unbounded acceleration to intro.}}. 

%This set considers all four combinations of initial and goal configurations speeds.


% Their algorithm solution cost is not much more than the optimal for the settings demonstrated, but there are no guarantees of the quality, or how far from the optimal the solution cost will be.

%For such systems, a minimum-time path can be computed in a similar fashion to the setting where no wind exists~\cite{minimum_time_const_wind}.
%However in this case, Dubins path has no analytical solution exists.
%Mittal et al.~\cite{Dubins_with_currents} used only two Dubins types~(RSR and LSL) to online-compute the path between two vehicles pose under ocean currents. 
%They did so because only those two have analytical expression.
%\DP{For such systems, the minimum-time can be computed in a similar fashion to the setting where no wind exists~\cite{minimum_time_const_wind}.
%However, in this case, only two Dubins types have analytical solution~(RSR and LSL).
%Mittal et al.~\cite{Dubins_with_currents} used those two to online-compute the path between two vehicles pose under ocean currents.}
%The second is adding a constraint that the system has bounds on the acceleration \DP{Add cite}. 
%For this case, no analytic solution exists for time-optimal motions. 
% \OS{DOUBLE CHECK WITH PETR AND GET SOME RELATED WORK}.

 
% In this paper we concentrate on search-based methods where the continuous search space~(space of all positions, orientations, and speeds) is discretized into a lattice, also called grid-based space, and search algorithms such as~\astar~\cite{hart1968formal} are used to compute a minimal-cost path.

%An extension for problems the aforementioned models aim to solve is the motion-planning problem for the case of multi-goal locations.
%With the number of the goal increase, the motion-planning problem becomes exponentially challenging.
%A known such problem is Dubins traveling salesman problem~(DTSP)~\cite{savla2008traveling} such as the work by~\cite{faigl2017solution}.
%A scenario of multi-agent motion-planning~\cite{kumar2012multi} becomes exponentially challenging as well with the number of agents.


% - problem.tex ---------------------------------------------------------------

   %, \quad u \in [-1, 1].


% We follow the formulation of the motion-planning problem as presented by Song et al.~\cite{T*}.

% We will start by describing the robotic-system dynamic.
% % The constant wind~$\vec{w} = (w_x, w_y)$. 
% % We denote~$\dot{\vec{x}}(t) = (\dot{x},\dot{y},\dot{\theta})^T$.
% The dynamics of the vehicle is defined by:
% % \begin{equation}
% %   \label{eq:dub}
% %   \dot{\vec{x}}(t) 
% %   = \left(
% %       \begin{array}{c}
% %      \dot{x} \\
% %      \dot{y} \\
% %      \dot{\theta} 
% %       \end{array}
% %   \right)
% %   =
% % %   f(\vec{x}(t), {v}(t), {u}(t))
% % %   =
% %   \left(
% %       \begin{array}{c}
% %      v \, \cos\,\theta \\
% %      v \, \sin\,\theta \\
% %      u
% %       \end{array}
% %   \right)
% % \end{equation}

% \begin{equation}
%     \begin{cases}
%     \dot{x}(t) = v(t) \cos\theta(t), \\
%     \dot{y}(t) = v(t) \sin\theta(t), \\
%     \dot{\theta}(t) = u(t).
%     \end{cases}
% \end{equation}
% Where~$(x,y,\theta) \in SE(2)$ and~$u, v$ are the control inputs.
% The first control input~$u$ controls the turn rate of the trajectory and is bounded according to the actual speed based on constant~$K$
% \begin{equation}
% |u| \leq \frac{K}{v}, u \in [-u _{\max},u _{\max}]
% \label{eq:curvature_limit}
% \end{equation}
%~$+/-$ refers to left/right turn. 
% A vehicle's speed is limited by its minimum and maximum speeds

% \begin{eqnarray}
%   v _{\min} \leq v \leq v _{\max} \\ \quad v _{\min} > 0 \\ \quad v _{\max} > 0
%   \label{eq:minmaxvel}
% \end{eqnarray}
% The robotic-system able to travel using two extreme radii:
% \begin{equation}
%     \rho_{max}=\frac{v _{\max}}{u _{\max}}.
% \end{equation}
% \begin{equation}
%     \rho _{\min}=\frac{v _{\min}}{u _{\max}}.
% \end{equation}
% This work assumes without losing generality that~$v _{\max}= 1$.

% Dubins's approach was generalized and the system configuration, also called configuration, is the four-dimensional vector~$s=(x,y,\theta,v)$, hence the configuration space is four-dimensional as well. 

% Let~$\mathcal{A}\subset\mathbb{R}^2$ be grid-based space where each cell in the grid is~$\mathcal{C} \in \{\mathcal{O}, \mathcal{F}\}$ where~$\mathcal{O}$ refers to cell which occupied by obstacle and~$\mathcal{F}$ refers to a free cell. 
% Let define the time-cost of collision-free path~$\gamma$ from the initial configuration~$s_{\text{start}}$ to the goal configuration~$s_{\text{goal}}$, as the integral over the path:
% \begin{equation}
%     P(\gamma) = \int_{\gamma} \frac{1}{v(p)}. dp
%     \label{eq:pathCost}
% \end{equation}
% Where~$v(p)$ refers to the vehicle speed at path segment~$dp$. 
% % We define a collision-free path~$\gamma$ as a configurations sequence from the initial configuration~$s_{\text{start}}$ to the goal configuration~$s_{\text{goal}}$ of~$P(\gamma)$, 
% Let denote the set of all collision-free paths as~$\Gamma$. 
% The time-optimal path~$\gamma^{*}$ is the path which has the least time-cost of all the paths from~$s_{\text{start}}$ to~$s_{\text{goal}}$, i.e~$P(\gamma^{*})~\leq~P(\gamma),\,~\forall \gamma \in \Gamma$.

% The objective is to find a sub-optimal path, represented by a set of consecutive configurations, from~$s_{\text{start}}$ to~$s_{\text{goal}}$ such that its time cost is not more than~$(1+\varepsilon)P(\gamma^{*})$ for~$\varepsilon~\geq~0,\,\varepsilon\in\mathbb{R}$.

% This work considers a scenario where each cell has eight optional orientations and each cell has eight neighbors.

% - background.tex ------------------------------------------------------------
% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}{.235\textwidth}
%         \includesvg[height=3cm]{pics/Map6_tstar_wo_wind.svg}
%         \caption{}
%          \label{fig:mutual_transitions-a}
%     \end{subfigure}
%     \begin{subfigure}{.235\textwidth}
%         \includesvg[height=3cm]{pics/minimum_speed_map_6.svg}
%         \caption{}
%          \label{fig:mutual_transitions-b}
%     \end{subfigure}
%     \begin{subfigure}{.235\textwidth}
%         \includesvg[height=3cm]{pics/mutual_transitions.svg}
%         \caption{}
%         \label{fig:mutual_transitions-c}
%     \end{subfigure}
%     \caption{
%     \protect
%     (\subref{fig:mutual_transitions-a})~The time-optimal solution obtained by~\tstar 
%     and
%     \protect
%     (\subref{fig:mutual_transitions-b})~the shortest path obtained by computing a Dubins path with minimum speed on the same setting.
%     Notice that both paths, which are in the same homotopy class, share many transitions.
%     % \protect
%     % (\subref{fig:mutual_transitions-c})~The percentage of transitions shared by the solution obtained by \tstar and by the shortest path out of the total number of transitions in~\tstar solution also found in the solution of Dubins path with minimum speed, vs. the number of configurations in~\tstar solution.
%     % % Each color refers to a different percentage of the map covered by obstacles.
%     % The average percentage of those mutual transitions in this evaluations of more than~$550$ experiments was almost~$89\%$.
%     \protect
%     (\subref{fig:mutual_transitions-c}).
%     The number of transitions in the solution $\gamma_{\tstar}$ obtained by~\tstar that also appear in the solution obtained by Dubins path of minimum speed as a function of the number of states in $\gamma_{\tstar}$. 
% %    The average of those mutual transitions in this evaluations of more than~$550$ experiments was almost~$89\%$
%     % Let denote~$T_{\tstar},T_{v_{\min}}$ as the sets of transitions in the paths found by~\tstar and Dubins path with minimum speed, respectively. In addition, let denote the mutual transitions set as~$T_{\text{mutual}} = \{T \vert T \in T_{\tstar} , T \in T_{\tstar} \cap T_{v_{\min}}\}$.
%     % \protect
%     % (\subref{fig:mutual_transitions-c})~shows~$\frac{n(T_{\text{mutual}})}{n(T_{\tstar})}$ vs. the number of configurations in~\tstar found path.
%     % The average of~$\frac{n(T_{\text{mutual}})}{n(T_{\tstar})}$ in this evaluations of more than~$550$ experiments was almost~$89\%$.
%     }
%     % \OS{caption and pic need some love. If page limitation is an issue---remove. Regardless, maybe add notation so (c) will be more formal. It is cumbersome now.}
    
% \label{fig:mutual_transitions}

% \end{figure*}


%and some insights on the computational complexity of it's different components.
%

%In addition to the two mentioned lists, the algorithm maintains a \textsc{Closed} list for the nodes that have already been expanded.

%at~$v_{\max}$ 

%and moving at maximum speed.

%\DP{As identified by~\cite{Wolek}, the optimal transition between configurations is one of~34 candidate. In this set, there are candidates that consider the options of start or reach the goal configuration either at minimum or maximum speed. We studied the case when a transition is computed for each speed in the start or goal configuration. Therefore, This work considers in this setting~68 unique transitions}. 

%\DP{length})\footnote{\DP{We have to make sure they are both measured in the same units. If we consider the time cost of Dubins path, it is larger than the time of time-optimal}} 

\ignore{

\tstar will be discussed here in detail and its important steps will be described.

% \begin{figure}[!t]
%     \centering
%     \begin{subfigure}{.235\textwidth}
%         \includesvg[width=1\linewidth]{pics/Map6_tstar_wo_wind.svg}
%         % {\includegraphics[scale=0.6]{pics/Lower bound quality}}
%         \caption{}
%     \end{subfigure}
%     \begin{subfigure}{.235\textwidth}
%         \includesvg[width=1\linewidth]{pics/minimum_speed_map_6.svg}
%         % {\includegraphics[scale=0.6]{pics/Lower bound quality}}
%         \caption{}
%     \end{subfigure}
%     \caption{The time-optimal solution is obtained by~\tstar~(a) and Dubins path with minimum speed~(b). 
%     % The robotic-system can travel either at minimum~(red) or maximum~(green) speed.
%     }
%     \label{fig:tstar_wo_wind}
% \end{figure}

% It finds a time-optimal risk-aware path. 
% This work considers only the time-optimal part and refers to~\tstar as time-optimal motion-planning algorithm for curvature-constrained robotic-systems.

The algorithm has based on the approach~\cite{Wolek} that finds an approximate solution for the time-optimal transitions between poses in the obstacle-free space.
This approach has been generalized by incorporating it into a motion-planning algorithm in grid-based space that also accounts for the risk of colliding with obstacles.
In our work, we refer to~\tstar as the version that optimizes time-optimal paths.

In grid-based space, there is a finite number of optional transitions between configurations.
Where each cell has eight optional orientations and eight neighbors, this number equal to~512.
Using symmetry and rotation, it can reduce to~68.

Using numerical nonlinear optimization and interior-point optimizer solver,~\texttt{IPOPT}~\cite{ipopt},~\tstar obtains an approximation for all possible time-optimal transitions between consecutive configurations.
From a robotics perspective, the optimization constraints are the robotic-system parameters, such as turning rate, the minimum velocity, and the maximum velocity. 
\astar-like search is then used to find a collision-free path that is time-optimal, referred to the set of calculated time-optimal transitions\footnote{The optimization algorithm is not guaranteed to find all the locally optimal paths, thus one cannot
conclude that the least-cost path is globally optimal.}, between the initial configuration~\start and the goal configuration~\goal.
They shown that the time-optimal path consist of segments in both minimum and maximum speed and its cost is lower than Dubins path either in minimum or maximum speed.

Pre-processing, where all the possible time-optimal transitions are calculated, requires significantly more computational resources than searching. 
The pre-processing optimizations last two orders of magnitude more than the search.
In practice, that means that the time-optimal optimizations last more than~$99\%$ of~\tstar runtime.
Furthermore, only a small fraction of all possible time-optimal transitions makes up an optimal path found by~\tstar.
% An example of time-optimal transitions in the solution of~\tstar can be seen in Fig.~\ref{fig:unique_transitions}. 
% Even for solutions with hundreds of configurations, the number of unique transitions in the solution does not change significantly. 
% This conclusion holds also for a different portion of the map which is occupied by obstacles.

The~\astar-like search is a best-first-search algorithm~\cite{best-first-search}.
In this type of algorithms, a graph search is built incrementally and it consists of vertices, also called nodes, and edges that connect the vertices.
% called in our case transitions between node's configurations. 
At each iteration, the algorithm decides which node will expand, i.e. which of its neighbors will gain a vertex.  It is assisted by a priority queue for this decision. 
Priority queue nodes are sorted by their~$f$ costs. 
The~$f$ cost of node~$n$ is the sum of~$g$ cost, which represents the path cost from~$s_{\text{start}}$ to the configuration of~$n$~(denote as~$n.\text{configuration}$), and~$h$ cost, which represent an assumption of the path cost from~$n.\text{configuration}$ to~$s_{\text{goal}}$.
In~\tstar, the heuristic cost~$h(n.\text{configuration},s_{\text{goal}})$ is determined by Dubins path using turning radius~$\rho _{\min}$ divided by maximum-speed~$v _{\max}$.
% Fig.~\ref{fig:tstar_wo_wind} shows an example of~\tstar solution. Fig.~\ref{fig:tstar_wo_wind}a shows the time-optimal path the algorithm found and Fig.~\ref{fig:tstar_wo_wind}b shows the time duration of each step of the algorithm. 
% It can be seen that the duration of time-optimal optimizations lasts much longer than the search step. Even though the time duration of the optimizations demands a long computational time, in static environment conditions the pre-processing can take place offline, and then its time duration can be ignored.

From our experience, in many settings, the time-optimal path, that is found by~\tstar, and the shortest path, that obtain by Dubins path in minimum speed, typically belong to the same homotopy class, i.e there is a continuous deformation between them without going through obstacles as can be seen in Fig.~\ref{fig:tstar_wo_wind}.
Furthermore, they often share a large portion of the transitions between consecutive configurations in the final path.
Fig.~\ref{fig:mutual_transitions} shows demonstrations of the mutual transitions in the~\tstar and Dubins path with minimum speed solution paths.
The y axis of the figure refers to the percentage of the transitions in~\tstar solution path that also found in the solution path of minimum speed Dubins.
% The average percentage of those mutual transitions in this demonstration of more than~$550$ experiments with varying obstacles portion coverage was almost~$89\%$. 
% Table~\ref{tab:transition_table} summarizes the solution configurations sequence of both shortest and the time-optimal, shown in Fig.~\ref{fig:tstar_wo_wind}.
% In eight orientations and eight neighbors setup, there are potentially 512 unique transitions but using rotation and symmetry these number reduces to~68.
% Each line in the table represents a trajectory between consecutive configurations and is described as:
% \begin{center}
%    ~$\underset{configuration_i}{(x_i,y_i,\theta_i)} \xrightarrow{} \underset{configuration_{i+1}}{(x_{i+1},y_{i+1},\theta_{i+1})}$ = Id of a transition
% \end{center}
% In eight neighbors and eight orientations for each cell setup, using rotation and symmetry, we can show that transitions that don't look same at first are actually the same. In addition, each transition can be considered as relative between~$configuration_i~$ and~$configuration_{i+1}$ as follows:
% Each transition can be considered as relative between~$configuration_i~$ and~$configuration_{i+1}$.
% Under translation and rotation, all transitions marked with the same id are equivalent.

% The calculation of the relative transitions is done by rotation, calculation of the relative position, and mirroring about the~$x$ axis or the~$x-y$ axis, depends on the orientation of the initial configuration.
% For rotation we can use standard rotation matrix:
% \begin{align}
% \label{eq:rotation_matrix}
%     R(\theta_{rot})= 
%     \begin{bmatrix} 
%     \cos \theta_{rot} & -\sin \theta_{rot} \\ \sin \theta_{rot} & \, \, \, \, \cos \theta_{rot}
%     \end{bmatrix}
% \end{align}

% \begin{equation}
%     \theta_{rot} =
%     \begin{cases}
%         -\theta_i, & (\theta_i) \bmod \frac{\pi}{2} = 0\\
%         -\theta_i + \frac{\pi}{4}, & else
%     \end{cases}
% \end{equation}

% After the rotation, the relative transition between~$configuration_i~$ and~$configuration_{i+1}$ is calculated as follows: 
% \begin{equation}
%     \begin{array}{l}
%         x_{relative} = x_{i+1}-x_i \\
%         y_{relative} = y_{i+1}-y_i \\
%         \theta_{relative} = (\theta_{i+1}-\theta_i) \bmod 2\pi
%     \end{array}
% \label{eq:transitions_formula}
% \end{equation}
% The mirror axis is determined by:

% \begin{equation}
%     \textup{mirror axis} =
%     \begin{cases}
%         x, & (\theta_i) \bmod \frac{\pi}{2} = 0\\
%         x-y, & else
%     \end{cases}
% \end{equation}

% We demonstrate it on the minimum speed Dubins column for rows 2 and 11. 
% For the transition in line 11 we first rotate both configuration by~$-\frac{\pi}{2}$ rad using~\ref{eq:rotation_matrix}:
% \begin{align}
%     R(-\frac{\pi}{2})
%     \begin{bmatrix}
%     4\\11
%     \end{bmatrix}
%     = 
%     \begin{bmatrix}
%     11\\-4
%     \end{bmatrix}
%     \\
%     R(-\frac{\pi}{2})
%     \begin{bmatrix}
%     3\\12
%     \end{bmatrix}
%     = 
%     \begin{bmatrix}
%     12\\-3
%     \end{bmatrix}
% \end{align}
% We did the same to the stats in line 2.
% It can be seen in table~\ref{tab:example} that by using~\ref{eq:transitions_formula} and mirroring about~$x-y$ axis, we get the same transition.

% \begin{figure}[!t]
%     \centering
%     % \adjustbox{margin=1em,width=\textwidth,set height=4cm,set depth=4cm,frame,center}{\includegraphics[scale=0.6]{pics/Lower bound quality}}
%     \includesvg[scale=0.55]{pics/mutual_transitions.svg}
%     % {\includegraphics[scale=0.6]{pics/Lower bound quality}}
%     \caption{The percentage of~\tstar solution transitions also found by Dubins path with minimum speed vs. the number of configurations in the solution path found by~\tstar. Each color refers to a different percentage of the map covered by obstacles.}
%     \label{fig:mutual_transitions}
% \end{figure}

% \begin{table}[!t]
% \renewcommand{\arraystretch}{2} % For vertical centering of the table
%             \centering
%             \begin{tabular}{|c|c|c|}
%                  \hline
%                  & \textbf{minimum speed Dubins} & \textbf{Time-Optimal}\\ [1ex]
%                 \hline
%                 \textbf{1} &~$(1,1,0) \rightarrow (2,2,\frac{\pi}{4}) = 1$ &~$(1,1,0) \rightarrow (2,2,\frac{\pi}{4}) = 1$\\
%                 \hline
%                 \textbf{2} &~$(2,2,\frac{\pi}{4}) \rightarrow (3,3,\frac{\pi}{2}) = 2$ &~$(2,2,\frac{\pi}{4}) \rightarrow (3,3,\frac{\pi}{2}) = 2$\\
%                 \hline
%                 \textbf{3} &~$(3,3,\frac{\pi}{2}) \rightarrow (3,4,\frac{\pi}{2}) = 3$ &~$(3,3,\frac{\pi}{2}) \rightarrow (3,4,\frac{\pi}{2}) = 3$\\
%                 \hline
%                 \textbf{4} &~$(3,4,\frac{\pi}{2}) \rightarrow (3,5,\frac{\pi}{4}) = 4$ &~$(3,4,\frac{\pi}{2}) \rightarrow (3,5,\frac{\pi}{4}) = 4$\\
%                 \hline
%                 \textbf{5} &~$(3,5,\frac{\pi}{4}) \rightarrow (4,6,\frac{\pi}{2}) = 2$ &~$(3,5,\frac{\pi}{4}) \rightarrow (4,6,\frac{\pi}{2}) = 2$\\
%                 \hline
%                 \textbf{6} &~$(4,6,\frac{\pi}{2}) \rightarrow (4,7,\frac{\pi}{2}) = 3$ &~$(4,6,\frac{\pi}{2}) \rightarrow (4,7,\frac{\pi}{2}) = 3$\\
%                 \hline
%                 \textbf{7} &~$(4,7,\frac{\pi}{2}) \rightarrow (4,8,\frac{\pi}{4}) = 4$ &~$(4,7,\frac{\pi}{2}) \rightarrow (5,8,\frac{\pi}{4}) = 6$\\
%                 \hline
%                 \textbf{8} &~$(4,8,\frac{\pi}{4}) \rightarrow (5,9,\frac{\pi}{2}) = 2$ &~$(5,8,\frac{\pi}{4}) \rightarrow (5,9,\frac{\pi}{2}) = 7$\\
%                 \hline
%                 \textbf{9} &~$(5,9,\frac{\pi}{2}) \rightarrow (5,10,\frac{\pi}{2}) = 3$ &~$(5,9,\frac{\pi}{2}) \rightarrow (5,10,\frac{\pi}{2}) = 3$\\
%                 \hline
%                 \textbf{10} &~$(5,10,\frac{\pi}{2}) \rightarrow (4,11,\frac{3\pi}{4}) = 1$ &~$(5,10,\frac{\pi}{2}) \rightarrow (4,11,\pi) = 8$\\
%                 \hline
%                 \textbf{11} &~$(4,11,\frac{3\pi}{4})\rightarrow (3,12,\frac{\pi}{2}) = 2$ &~$(4,11,\pi)\rightarrow (3,12,\frac{\pi}{2}) = 8$\\
%                 \hline
%                 \textbf{12} &~$(3,12,\frac{\pi}{2})\rightarrow (2,12,\frac{3\pi}{2}) = 5$ &~$(3,12,\frac{\pi}{2})\rightarrow (2,12,\frac{3\pi}{2}) = 5$\\
%                 \hline
%             \end{tabular}
%             \caption{configurations sequences of the solutions of minimum speed Dubins and time-optimal motion-planning.}
%             \label{tab:transition_table}
% \end{table}

% \begin{table}[!b]
% \renewcommand{\arraystretch}{2} % For vertical centering of the table
%         \centering
%         \begin{tabular}{|c|c|}
%             \hline
%             \textbf{Row 2} & \textbf{Row 11}\\ [1ex]
%             \hline
%            ~$x_{relative} = 1$ &~$x_{relative} = 1$\\
%            ~$y_{relative} = 1$ &~$y_{relative} = 1$\\
%            ~$\theta_{relative} =+\frac{\pi}{4}$ &~$\theta_{relative} =-\frac{\pi}{4}$\\
%             \hline
%         \end{tabular}
%     \caption{configurations transition example.}
%     \label{tab:example}
% \end{table}
% In this scenario, the shortest and time-optimal paths share a significant part of their transitions in the solution.
% The ids were chosen arbitrarily. 
%~\tstareps uses those transitions to estimate which transitions would be a part of a sub-optimal solution, and in that way, reduces the number of time-optimal optimizations and reduces the algorithm's runtime. 

In dynamic environment conditions, pre-processing can not take place. In presence of wind for example, if time-optimal transitions are not calculated for specific wind conditions, it can not guarantee that the solution path will be collision-free and not even that the robotic-system reaches its goal.

This work aims to solve the time-optimal curvature-constrained motion-planning more efficiently when balancing between runtime and solution quality, especially in change environmental conditions when an offline pre-processing can not be done.
%  The solution of~\tstar defined a path from the start to the target configuration with less time cost compared to the calculated Dubins paths using uniformly either the minimum or maximum velocity.

% \begin{figure}[!b]
%     \centering
%     % \adjustbox{margin=1em,width=\textwidth,set height=4cm,set depth=4cm,frame,center}{\includegraphics[scale=0.6]{pics/Lower bound quality}}
%     \includesvg[scale=0.45]{pics/Map6_tstar_wo_wind.svg}
%     % {\includegraphics[scale=0.6]{pics/Lower bound quality}}
%     \caption{Time-optimal solution obtained by~\tstar. The robotic-system can travel either in minimum (red) or maximum (green) speed.}
%     \label{fig:tstar_wo_wind}
% \end{figure}
}

% - method.tex ----------------------------------------------------------------

% In this section, we present a novel bounded-suboptimal minimum-time motion-planning algorithm, called~\tstareps, for curvature-constrained systems that aims to find a solution with significantly less runtime compared to the computational time the optimal solution requires and with an upper-bound on the solution quality.

% Since the problem domain is grid-based space, it can be determined that:~(i) there are a finite number of optional time-optimal transitions between consecutive configurations and~(ii) finding approximations for time-optimal transitions, and the search algorithm can be performed independently. 
% In addition, as mentioned at~\ref{sec:alg background} the search requires a much smaller computational effort compared to the optimizations. 

% \tstareps algorithm suggests a novel approach that uses the connection between the shortest and time-optimal paths. 
% This connection is reflected in the fact that the shortest and time-optimal paths usually share the same homotopy class and most of the transitions between configurations in their solutions. 
% The shortest path can be found very easily, using Dubins path, and in a short computational time. 
% The search algorithm we use is based on~\astar algorithm and is specifically inspired by~\astareps~\cite{astareps}.

% ~\astar, and its variants, are best-first-search algorithms where the search graph is incrementally built as described in~\ref{sec:alg background}.


%~\astar, and its variants, are best-first-search algorithms where the search graph is incrementally built as described in~\ref{sec:alg background}.
% Since time-optimal optimizations are computationally expensive,~\tstareps aims to perform a few of them as possible.
% Therefore, during the graph's expansion, each edge added can be set either with its true time-optimal cost, which requires high computation effort, or with a lower bound of the true cost.
% Researchers investigated and proved that using lower bounds for especially expensive to evaluate edges in graphs is efficient.
% This technique also knows as lazy search~\cite{lazy_search}.
% It is possible to select a lower bound considering or not the presence of obstacles, the curvature-constrained distance, or the Euclidean distance.
% The lower bound has to be both optimistic, i.e its cost will be smaller than the real cost, and as informative, i.e its cost should be \textsc{Closed} to the real cost. 
% The closer the lower bound is to the true cost, the fewer total expansive edge evaluations, i.e calculating time-optimal transitions,  will exist. 
% It also should be computationally cheaper to evaluate.
% % It is important that a lower bound cost is less than the real cost, be as informative as possible, and be computationally cheaper to evaluate.
% lower bound options will be discussed in detail in~\ref{sec:results}.

%Recall (Sec.~\ref{sec:problem} and Sec.~\ref{sec:alg background}) that we consider a discretized search space with a finite set of possible transition types in this space.
%

%denote the cache table as~$\mathcal{C}$, 
%\DP{Denote with~$\mathcal{C}[T]$ the action of caching in/out the true cost of already computed transition~$T$.}

%will be clear when we describe how it is used to order nodes lexicographically in the \textsc{Focal} list where lower will be better.}

   % ~\ForAll{$s \leftarrow \texttt{\textup{find\_all\_successors(}}n\texttt{)}$}{
   % \text{use Eq.~\ref{eq:g-value} to evaluate its~$g$-value}\\
   % }
   % ~~\If{incoming transition~$n.T$ was not expanded ($\kappa (n.T) = 1$)} { 
   %     compute~$c(n.T)$, cache result and set~$\kappa = 0$
   %     }
   % ~~for every succesor node~$n'$, use Eq.~\ref{eq:g-value} to evaluate its~$g$-value.

% \begin{algorithm}[!t]
% \color{red}
% \caption{\text{\boldtstareps}}
% \label{alg:tstar-eps}
% \KwIn{$\text{map}, \mathbf{s}_\text{start}, \mathbf{s}_\text{goal}, \text{approximation factor}\, \varepsilon$}
% \KwOut{$\text{path from}~$~$\mathbf{s}_\text{start}\, \text{to}\, \mathbf{s}_\text{goal}$}
% %
% \vspace{2mm}
% %
% \noNumber{\color{blue} 
% \texttt{\textbf{S1.}~compute~$c()$ for an initial path}}
% %
%  ~$\gamma_{\text{SP}}^{v_{\min}} \leftarrow$ Dubins path on map using~$v_{\min}$ \label{tstareps-shortest} \\
% %
%   \textbf{for each} transition~$T \in \gamma_{\text{SP}}^{v_{\min}}$ \textbf{do} \label{tstareps-for_each_transition}\\ 
%   ~~compute~$c(T)$, cache result %$\mathcal{C}[T]$ 
%   and set~$\kappa(T) = 0$ \label{tstareps-update_kappa}\\
% %
% \vspace{2mm}
% %
% \noNumber{\color{blue} 
% \texttt{\textbf{S2.}~\astareps-like search}}
% %
% run \astareps nodes in \textsc{Focal} ordered by Eq.~\ref{eq:focal-key} \label{tstareps-astareps}\\
% %$n \leftarrow \texttt{find\_next\_node(\textsc{Open})}$ \label{tstareps-find_next}\\
% \textbf{when} expanding a node~$n$ \textbf{do}\\
% %
% ~~\textbf{if}{  $\kappa (n.T) = 1$} \textbf{then}\\
% \tcp{\footnotesize incoming transition~$n.T$ was not computed}\\
% ~~~~compute~$c(n.T)$ and set~$\kappa(n.T) = 0$\\
% %~~~~\DP{\textbf{continue to next iteration}} \\
% %
% ~~\textbf{if}{ node~$n$ is~$s_{\text{goal}}$} \textbf{then}\\
% ~~~~\textbf{return} path associated with~$n$\\
% %
% ~~\textbf{for each} succesor node~$n'$ of~$n$ in map \textbf{do} \DP{\tcp{\footnotesize expansion of node~$n$}}
% ~~~~~use Eq.~\ref{eq:g-value} to evaluate the~$g$-value of~$n'$ \label{tstareps-set_g} 
% \ignore{
% \textbf{if} incoming transition~$n.T$ was not expanded ($\kappa (n.T) = 1$) \textbf{then}\label{tstareps-expanding_n}\\
% ~compute~$c(n.T)$, cache result and set~$\kappa = 0$\
% %
% % ~$\text{Succ(}n\text{)} \leftarrow \forall n', n'.\text{parent}=n$\\
% ~\textbf{for each} successor~$n'$ of~$n$ \textbf{do} \\
% ~~use Eq.~\ref{eq:g-value} to evaluate its~$g$-value,~$n'.g$ \label{tstareps-set_g} \\}
% % ~\ForAll{$s \leftarrow \texttt{\textup{find\_all\_successors(}}n\texttt{)}$}{
% % \text{use Eq.~\ref{eq:g-value} to evaluate its~$g$-value}\\
% % }
% % ~~\If{incoming transition~$n.T$ was not expanded ($\kappa (n.T) = 1$)} { 
% %     compute~$c(n.T)$, cache result and set~$\kappa = 0$
% %     }
% % ~~for every succesor node~$n'$, use Eq.~\ref{eq:g-value} to evaluate its~$g$-value.
% \end{algorithm}

% \begin{equation}
% \label{eq:g-value}
%  n.g = n.\text{parent}.g + 
%  \begin{cases}
%   \hat{c}(n.\text{T})  \text{~if~} \kappa(n.\text{T})=1,\\    {c}(n.\text{T})  \text{~if~} \kappa(n.\text{T})=0.
%  \end{cases}
% \end{equation}

% \DP{
% \begin{equation}
% \label{eq:f-value}
%     n.f = g(n) + h(n).
% \end{equation}
% }
% Here,~$h(n)$ can be any admissible estimate of the cost to reach the goal.
% In our setting we use the length of minimum speed Dubins path divided by the vehicle's maximum speed.
%
% \DP{
% \begin{equation}
% \label{eq:focal-key}
%     \text{key}(n) = (\kappa(n.T) , n.f).
% \end{equation}
% }

% \DP{
% According to Cor.~\ref{cor:subpot}, any choice of a node to expand from~\textsc{Focal} leads to a solution cost that is not greater than the optimal by more than~$1+\varepsilon$.
% Hence in \tstareps, only nodes whose true cost has already been computed are expanded.
% }

\ignore{
\DP{
As mentioned, \textbf{S2} is~\astareps-like search.
Here we describe only the non-generic part of it in~\tstareps.
This part consists of two components, how~\tstareps decides which node to expand~(line~\ref{tstareps-find_next}) and how it computes~$g$-value for the successors of expanded node~(line~\ref{tstareps-set_g_value}).
}

\DP{
Algorithm~\ref{alg:find-next_focal} explains how~\tstareps decides which node to expand. First it verifies if the~\textsc{Focal} list is not empty. 
If it is, the algorithm returns that there is not solution for the problem~(lines \ref{find-next_focal_empty}-\ref{find-next_go_out}).
This check is important since there are guarantees that after computation of a new transition~(lines \ref{find-next_top_open}-\ref{find-next_try_again}) the~\textsc{Open}, and accordingly the~\textsc{Focal}, will not be empty.  
% The importance of this check will be explained.
If the~\textsc{Focal} is not empty and the transition's true cost of the node in the top of it have already been computed, the algorithm pop and returns this node, denoted as~$n_{\text{focal}}$~(lines \ref{find-next_top_focal}-\ref{find-next_return_top}).
In the case there is no node in the focal that its true cost have already been computed, the algorithm computes the true cost for the transition, denote as~$T_{\text{new}}$, of the node in the top of~\textsc{Open}, cache it and updates the~$\kappa$ value of~$T_{\text{new}}$~(lines \ref{find-next_top_open}-\ref{find-next_update_kappa}).
It repeats the procedure until the condition at line~\ref{find-next_check_focal_top} is met~(line~\ref{find-next_try_again}).
% After the new transition is computed, the~\textsc{Open}, and accordingly the~\textsc{Focal}, can be empty. 
% For example, in a situation there was only one node in~\textsc{Open} and its transition computation returns no solution, the numerical evaluation does not converge, it considers as not collision-free and therefore removed from~\textsc{Open}.
% In this case, those two lists have no nodes and it means there is no solution for the problem.
% Here comes the importance of lines~\ref{find-next_focal_empty}-\ref{find-next_go_out}.
}}

% \DP{
% In our setting , each node~$n$ considered by the search 
% is associated with a parent node~$n.\text{parent}$,
% the~$f$-value which is:
% \begin{equation}
% \small
%     n.f = 
%     \begin{cases}
%     g(n.\text{parent)} + \hat{c}(n.\text{T}) + h(n), \; \kappa(n.\text{T})=0,\\
%     \underbrace{g(n.\text{parent)} + c(n.\text{T})}_{n.g} + h(n), \; \kappa(n.\text{T})=1.
%     \end{cases}
% \end{equation}
% These are standard in \astareps and in our setting we also associate the minimial-time transition~$n.\text{T}$ that was used to move the system from the configuration associated with~$n.\text{parent}$ to the configuration associated with~$n$.
% Since use the~\textsc{Focal} guarantees~$1 + \varepsilon$ optimality for any choose of node, in our case the \textsc{Focal} consist of only node their transitions true costs have already been computed:
% \begin{equation}
% \scriptsize	
%     \textsc{Focal} = \left\{ \text{n} \in \textsc{Open} \mid  f(n) \leq (1+\varepsilon) \underset{\textup{n'}\in \textsc{Open}}{\min} f(\textup{n'}),~\kappa(\text{n.T})=1 \right\}.
%     \label{eq:focal}
% \end{equation}

% }

% \DP{
% This is a best-first-search algorithm~\cite{best-first-search}.
% In this type of algorithms, a graph search is built incrementally and it consists of vertices, also called nodes, and edges that connect the vertices.
% % called in our case transitions between node's configurations. 
% At each iteration, the algorithm decides which node will be expanded, i.e. which of its neighbors will gain a vertex.  It is assisted by a priority queue for this decision. 
% Priority queue nodes are sorted by their~$f$ costs. 
% The~$f$ cost of node~$n$ is the sum of~$g$ cost, which represents the path cost from~$s_{\text{start}}$ to the configuration of~$n$~(denote as~$n.\text{configuration}$), and~$h$ cost, which represent an assumption of the path cost from~$n.\text{configuration}$ to~$s_{\text{goal}}$.
% }

% \DP{
% The algorithm runs as long as the~\textsc{Open} is not empty~(line~\ref{tstareps-check_open}).
% It finds the next node to expand~(line~\ref{tstareps-find_next}), removes it from the~\textsc{Open} and adds it to the~\textsc{Closed}~(lines~\ref{tstareps-open-next}-\ref{tstareps-closed+next}).
% If the configuration of next is the goal configuration, it returns the found sub-optimal path from~\start to~\goal~(lines~\ref{tstareps-check_next_is_goal}-\ref{tstareps-return_path}).
% For each successor~$s$ of next's configuration, the cost of the path between them is calculated and added to the~$g$-value of next for calculate the~$g$-value of a new crated node, denoted as~$n_{\textup{new}}$~(line \ref{tstareps-new_g}).
% As done in standard~\astar search, the algorithm determines whether a node with the successor's configuration already explored or expanded.
% % If such node exist, the algorithm determined if the cost from~\start to the successor's configuration is cheaper than the already found~(reflected by the~$g$-value of both nodes). 
% If such node exist, the algorithm determines if its cost-to-come is cheaper than the already found. 
% If this is the case, it updates the~\textsc{Open} and/or the~\textsc{Closed} accordingly~(lines~\ref{tstareps-old_in_open}-\ref{tstareps-add_new_to_open}).
% % The algorithm determines if the configuration~$s$ already explored, i.e there is a node in \textsc{Open} that his configuration is~$s$~(line~\ref{tstareps-find_old_in_open}). 
% % If such node is found, denote as~$n_{\textup{old}}$, the algorithm checks which node has lower~$g$ cost that indicates on a path with least cost from~\start to~$s$.
% % If the new node has a cheaper cost than the algorithm updates~$n_{\textup{old}}$~(lines~\ref{tstareps-old_in_open}-\ref{tstareps-update_open_old}).
% }
% \DP{
% % If there is no node in \textsc{Open} such that its configuration is~$s$, it determines if there is such node in \textsc{Closed}~(line~\ref{tstareps-find_old_in_closed}) and repeats the evaluation it did in lines~\ref{tstareps-old_in_open}-\ref{tstareps-update_open_old}.
% % If the new node has cheaper path cost from~\start to~$s$,~$n_{\textup{old}}$ is updated, it is removed from the~\textsc{Closed} list, and added to the \textsc{Open} list~(lines~\ref{tstareps-closed-old}-\ref{tstareps-open+old}).
% % If the configuration~$s$ doesn't belong to any node either in \textsc{Open} and \textsc{Closed}, the algorithm calculates its fields to the new node and adds the node to the \textsc{Open} list~(lines~\ref{tstareps-set_new_parent}-\ref{tstareps-add_new_to_open}).
% }

% \DP{
% % During the search, the algorithm maintains \textsc{Open} list for all the nodes that have been explored but not been expanded and \textsc{Closed} list for all expanded nodes. 
% The found path is configurations sequence of expanded nodes, which means that all of them are in the \textsc{Closed} list. 
% Moreover, the found sub-optimal path~$\gamma_{_{\tstareps}}$ includes configurations such that the true costs of the transitions between them were computed,~$\forall T \in \gamma_{_{\tstareps}},~\kappa(T)=1$. 
%  Thus, only nodes whose the true cost of their transition already computed are expanded during the search algorithm. 
% In each~\tstareps iteration, the algorithm uses a~\textsc{Focal} list to decide which node to expand.
% }

% \begin{equation}
% \scriptsize	
%     \textsc{Focal} = \left\{ \text{n} \in \textsc{Open} \mid  f(n) \leq (1+\varepsilon) \underset{\textup{n'}\in \textsc{Open}}{\min} f(\textup{n'}),~\kappa(\text{n.T})=1 \right\}.
%     \label{eq:focal}
% \end{equation}
% \DP{
% Where~\text{n.T} denote the transition between n node's parent and configuration. 
% }
% \DP{
% Following~{\bfseries{Theorem 1}} in~\cite{astareps}, for reasons of space we will not detail the proof in full.
% \begin{lemma}
% For any user defined~\eps,~\tstareps is~\eps-admissible, i.e., it always finds a solution
% whose cost does not exceed the optimal cost by more than a factor~$1+\varepsilon$ the optimal,~$\gamma_{_{\tstar}}$.
% \end{lemma}
% \begin{equation}
%     \gamma_{_{\tstareps}}\leq (1+\varepsilon)\gamma_{_{\tstar}}.
% \end{equation}
% }
% if during the search only nodes from the \textsc{Focal} are expanded, the cost of the found path is not more than~$1+\varepsilon$ of the optimal. This work aims to reduce computational time, so as long as the upper bound of the solution quality is guaranteed, any heuristic can be used to select nodes for expansion, even inadmissible ones. 
% As far as possible, this heuristic aims to reuse transitions that have already been computed. Therefore, nodes with already computed transition true costs are prioritized for expansion.

% \DP{
% Alg.~\ref{alg:find-next_focal} summarizes the procedure for finding the next node to expand~(Alg~\ref{alg:tstar-eps} line~\ref{tstareps-find_next}).
% The algorithm checks whether there is any node in~\textsc{Focal} and returns the node with the lowest~$f$-value in this list~(lines~\ref{find-next_check_focal}-\ref{find-next_return_argmin}). If this list is empty, it first determines whether the \textsc{Open} list is not empty. 
% In the case of empty \textsc{Open}, the algorithm returns that there is no solution for the problem~(lines~\ref{find-next_open_empty}-\ref{find-next_go_out}).
% In the case the~\textsc{Open} is not empty, it computes the true cost of the transition of the node in the top of the \textsc{Open} list and its predecessor, denote as~$T_\textup{new}$, cache it and marks this transition as computed(line~\ref{find-next_top_open}-\ref{find-next_update_kappa}).
% It repeats the procedure until the condition at line 1 is met~(line~\ref{find-next_try_again}).
% }

% \DP
% {
% As mentioned above, in best-first-search algorithms each node~$n$ has~$g$ cost that represents the cost from~\start to~$n.\text{configuration}$. Specifically, the~$g$ cost consists of two components:~(i) the~$g$ cost of~$n.\text{parent}$ and~(ii) the cost of the transition from~$n.\text{parent}$ to~$n.\text{configuration}$, denote this transitions as~$T_{n.\text{parent}}^{n.\text{configuration}}$.
% }

% \DP{
% Algorithm~\ref{alg:cost_func-kappa} summarizes the calculations to determines the~$g$-value of new node in~\tstareps. %~(algorithm~\ref{alg:astareps-like} line~6). 
% The algorithm determines if the true cost of the transition is already computed~(line~\ref{cost_func-k_value}). 
% If this is the case, the true cost of it is cached out and returned~(line~\ref{cost_func-true_cost}). 
% Otherwise, a lower bound for the true cost of the transitions is returned~(line~\ref{cost_func-lower_bound}). 
% }

% \begin{algorithm}[!t]
% \caption{\text{\tstareps}}
% \label{alg:tstar-eps}
% \KwIn{$\text{map}, \mathbf{s}_\text{start}, \mathbf{s}_\text{goal}, \text{approximation factor}\, \varepsilon$}
% \KwOut{$\text{bounded-suboptimal  minimum-time path from}~$\\~$\mathbf{s}_\text{start}\, \text{to}\, \mathbf{s}_\text{goal}$}
% % Ask Oren to use path or trajectory.
% %\BlankLine
% %
% \noNumber{\color{blue} \texttt{\textbf{S1}-computing~$c()$ for some transitions}}
% %
%~$\gamma_{\text{SP}}^{v_{\min}} \leftarrow  \text{Dubins\,path}(v_{\min})$\label{tstareps-shortest} \\
% \ForAll{$T \in \gamma_{\text{SP}}^{v_{\min}}$\label{tstareps-for_each_transition}}
% {
%~$\mathcal{C}[T] \leftarrow c(T)$ \label{tstareps-compute_transitions} \\
%~$\kappa(T) \leftarrow 1$ \label{tstareps-update_kappa} \\
% }
% %
% \noNumber{\color{blue} \texttt{\textbf{S2}-\astareps-like search}}
% %
% \While{$\textsc{Open} \neq \emptyset$ \label{tstareps-check_open}}{
%   ~$\text{next} \leftarrow \texttt{find\_next\_node(\textsc{Open})}$ \label{tstareps-find_next} \\ 
%   ~$\textsc{Open} \leftarrow \textsc{Open} \setminus\text{next}$ \label{tstareps-open-next}\\
%   ~$\textsc{Closed} \leftarrow \textsc{Closed} \cup \text{next}$ \label{tstareps-closed+next}\\
%       \uIf{$\texttt{\textup{is\_goal}}\textup{(next)}$\label{tstareps-check_next_is_goal}}{
%         \KwRet \textup{sub-optimal path from~$\mathbf{s}_\text{start}\, \text{to}\, \mathbf{s}_\text{goal}$ \label{tstareps-return_path}}
%     }
%     \For{$\text{s} \in \textup{succ(next})$ \label{tstareps-next_childs}}{
%         %$\text{cost\_to\_s} \leftarrow \texttt{cost(next.configuration,s)}$ \label{tstareps-cost_func}\\
        
%       ~$n_{\textup{new}}.g \leftarrow \text{next}.g + \texttt{cost(next,s)}$ \label{tstareps-new_g}\\
%         %\text{cost\_to\_s}$ 
        
         
%         \uIf{
%       ~$n_{\textup{old}} \leftarrow \texttt{\textup{find\_configuration(s,\textsc{Open})}}$
%         %$n_{\textup{old}
%         \label{tstareps-old_in_open}}{
%             \uIf{$n_{\textup{new}}.g < n_{\textup{old}}.g$\label{tstareps-new_is_better_open}}{
%                 \text{update}~$n_{\textup{old}}$\label{tstareps-update_open_old}\\
%                 %~$n_{\textup{old}}.g \leftarrow n_{\textup{new}}.g$\\
%                 %~$n_{\textup{old}}.parent \leftarrow \textup{next}$\\
%                 %~$n_{\textup{old}}.f \leftarrow n_{\textup{old}}.g + n_{\textup{old}}.h$\\
%             }
%         }
%         \uElse{
%             \uIf{$n_{\textup{old}} \leftarrow \texttt{\textup{find\_configuration(s,\textsc{Closed})}}$}{
%                     \uIf{$n_{\textup{new}}.g < n_{\textup{old}}.g$ \label{tstareps-new_is_better_closed}}{
%                     \text{update}~$n_{\textup{old}}$ \label{tstareps-update_closed_old}\\
%                     %~$n_{\textup{old}}.g \leftarrow n_{\textup{new}}.g$\\
%                     %~$n_{\textup{old}}.parent \leftarrow \textup{next}$\\
%                     %~$n_{\textup{old}}.f \leftarrow n_{\textup{old}}.g + n_{\textup{old}}.h$\\
%                   ~$\textsc{Closed} \leftarrow \textsc{Closed} \setminus n_{\textup{old}}$ \label{tstareps-closed-old}\\
%                   ~$\textsc{Open} \leftarrow \textsc{Open} \cup n_{\textup{old}}$ \label{tstareps-open+old}\\}
%             }
%             \uElse{
%                   ~$n_{\textup{new}}.parent \leftarrow \textup{next}$ \label{tstareps-set_new_parent}\\
%                   ~$n_{\textup{new}}.f \leftarrow n_{\textup{new}}.g + h(s)$ \label{tstareps-set_new_f}\\
%                   ~$\textsc{Open} \leftarrow \textsc{Open} \cup n_{\textup{new}}$ \label{tstareps-add_new_to_open}}
%             }
%         }
%         %~$\text{s.f} = \textup{next.g} + \text{cost\_to\_s} + \text{h(s)}$\\
%         % \If{$\text{s} \in \textup{OPEN or } \text{s} \in \textsc{Closed}$}
%         % {
%         %     \text{Check if s the current path to~$s$ is better} \newline \text{than the one already found and} \newline \noindent \text{update \textsc{Open} and \textsc{Closed}}
%         % }
%     }
% \end{algorithm}

\ignore{
\begin{algorithm}[!t]
\caption{\text{\tstareps}}
\label{alg:tstar-eps}
\KwIn{$\text{map}, \mathbf{s}_\text{start}, \mathbf{s}_\text{goal}, \text{approximation factor}\, \varepsilon$}
\KwOut{$\text{bounded-suboptimal  minimum-time path from}~$\\~$\mathbf{s}_\text{start}\, \text{to}\, \mathbf{s}_\text{goal}$}
%
\noNumber{\color{blue} 
\texttt{\textbf{S1.}~compute~$c()$ for some transitions}}
%
 ~$\gamma_{\text{SP}}^{v_{\min}} \leftarrow$  minimal-length collision-free Dubins path on map using~$v_{\min}$ \\
%
  \textbf{for each} transition~$T \in \gamma_{\text{SP}}^{v_{\min}}$, 
  compute~$c(T)$, cache result and set~$\kappa = 0$\\
%
%
\noNumber{\color{blue} 
\texttt{\textbf{S2.}~\astareps-like search}}
%
run \astareps with nodes in \textsc{Open} and \textsc{Focal} ordered according to Eq.~\ref{eq:f-value} and~\ref{eq:focal-key}, respectively \label{tstareps-astareps}\\
%
\textbf{when} expanding a node~$n$ \textbf{do}\\
%
~~\If{incoming transition~$n.T$ was not expanded ($\kappa (n.T) = 1$)} { 
    compute~$c(n.T)$, cache result and set~$\kappa = 0$
    }
~~for every succesor node~$n'$, use Eq.~\ref{eq:g-value} to evaluate its~$g$-value.
\end{algorithm}







\begin{algorithm}[!t]
\caption{\text{\tstareps}}
\label{alg:tstar-eps}
\KwIn{$\text{map}, \mathbf{s}_\text{start}, \mathbf{s}_\text{goal}, \text{approximation factor}\, \varepsilon$}
\KwOut{$\text{bounded-suboptimal  minimum-time path from}~$\\~$\mathbf{s}_\text{start}\, \text{to}\, \mathbf{s}_\text{goal}$}
% Ask Oren to use path or trajectory.
%\BlankLine
%
\noNumber{\color{blue} \texttt{\textbf{S1}-computing~$c()$ for some transitions}}
%
$\gamma_{\text{SP}}^{v_{\min}} \leftarrow  \text{Dubins\,path}(v_{\min})$\label{tstareps-shortest} \\
\ForAll{$T \in \gamma_{\text{SP}}^{v_{\min}}$\label{tstareps-for_each_transition}}
{
$\mathcal{C}[T] \leftarrow c(T)$ \label{tstareps-compute_transitions} \\
$\kappa(T) \leftarrow 0$ \label{tstareps-update_kappa} \\
}
%
\noNumber{\color{blue} \texttt{\textbf{S2}-\astareps-like search}}
%
run \astareps with nodes in \textsc{Open} ann \textsc{Focal} ordered according to Eq.~\ref{eq:f-value} and~\ref{eq:focal-key}, respectively \label{tstareps-astareps}\\
% \While{$\textsc{Open} \neq \emptyset$ \label{tstareps-check_open}}{
 ~$\text{next} \leftarrow \texttt{find\_next\_node(\textsc{Open})}$ \label{tstareps-find_next} \\ 
  \ForAll{$\text{n'} \in \textup{succ(next})$ \label{tstareps-next_childs}}{
       ~$\text{compute n'.} g \text{ using Eq.~\ref{eq:g-value} and n'.T}$ \label{tstareps-set_g_value}\\
        %~$\text{cost\_to\_s} \leftarrow \texttt{cost(next.configuration,s)}$ \label{tstareps-cost_func}\\
    }
% }
\end{algorithm}
}

% The algorithm has three main steps:~(i) First, it finds the shortest path from~$s_{\text{start}}$~to~$s_{\text{goal}}$ using Dubins path with minimum speed.~(ii) It computes true cost for transitions that appeared in the solution of~(i).~(iii) It performs~\astareps-like search to find a sub-optimal path from~$s_{\text{start}}$~to~$s_{\text{goal}}$ which its cost is not more than~\eps times the cost of an optimal path.

% \begin{enumerate}[A.] 
%     \item \textit{Finding the shortest path from~$s_{\text{start}}$ to~$s_{\text{goal}}$} \\
%      As mentioned above, the time-optimal, that is found by~\tstar, and the shortest paths typically belong to the same homotopy class and often share a large portion of the transitions between consecutive configurations in the final path.
     
%      Furthermore, the computational cost requires to finding the shortest path using Dubins path is negligible compare to computation of time-optimal transitions.  
    
%     % The algorithm uses this connection between the time-optimal and the shortest paths to reduce the most computationally expensive component, time-optimal optimizations.
%     % The shortest path allows us to determine which  time-optimal transitions are likely to be part of the sub-optimal solution. 
%     % Finding shortest paths by using Dubins path is much cheaper compared to the computation needed for time-optimal optimizations. 
    
%     An additional benefit comes from the shortest path search at the beginning of the algorithm. If no solution exists for the shortest path problem, then there is also no sub-optimal solution to the time objective problem. The algorithm is complete, i.e finds a solution if there is one. When compared to the optimal solution, which requires a lengthy optimization process, the shortest path can be found in a very short time.\footnote{\DP{Consider to remove.}}
    
%     As a result, if the sub-optimal minimum-time problem does not have a solution, it can be found without spending a significant amount of time.
    
%     \item \textit{Calculate an initial set of time-optimal transitions} \\
%     Having found the shortest path, the algorithm computes time-optimal for all the transitions who appeared in the shortest path solution.
%     % Transitions that were part of the shortest path are more likely to also be part of the time-optimal path. 
%     % During the search, the algorithm aims to calculate as few as possible time-optimal transitions and prefers to use configurations with already calculated such transitions.
%     During the search, the algorithm wish to re-use already computed time-optimal transitions.

    
%     \item \textit{\astareps-like search} \\
%     After the shortest path has been found and its solution transitions were computed, the algorithm searches for a sub-optimal path from~$s_{\text{start}}$ to~$s_{\text{goal}}$. 
%     % After he shortest path has been found and the most likely transitions are calculated, the algorithm searches for a sub-optimal path from~$s_{\text{start}}$ to~$s_{\text{goal}}$. 
%     % As mentioned above, the search is done using an~\astareps-like algorithm which is a best-first-search algorithm~\cite{best-first-search}. 
    
%     % In this type of algorithms, a graph search is built incrementally and it consists of vertices, also called nodes, and edges that connect the vertices. At each iteration, the algorithm decides which node will expand, i.e. which of its neighbors will gain a vertex.  It is assisted by a priority queue for this decision. Priority queue nodes are sorted by their~$f$ costs. The~$f$ cost of node~$n$ is sum of~$g$ cost, which represents the path cost from~$s_{\text{start}}$ to~$n$, and~$h$ cost, which represent an assumption of the path cost from~$n$ to~$s_{\text{goal}}$.
%     % As mentioned above, the search is done using an~\astareps-like algorithm.
    
%     Let denote two sets of transitions~$T_\text{opt}$ as the set of already computed true cost transitions, and~$T_\text{lb}$ as the set of transitions that their true cost was not calculated yet and their cost is defined by the lower bound of the true cost.
%     Any transition between configurations belongs to one of those sets.
%     In~\tstar all the transitions are belonged to~$T_\text{opt}$.
%     Let denote~$\mathcal{T}_\text{s}^\text{s'}$ as the transition from configuration s to s'.
     
%      In the search graph, each node~$n$ marked whether the true cost of the transition from its parent to its configuration already computed~$n.\text{transition}\in T_\text{opt}$, or not,~$n.\text{transition}\in T_\text{lb}$.
    
%     % Let denote two sets of edges.~$E_{\text{opt}}$, the set of true cost edges in the search graph, and~$E_{\text{low}}$, the set of lower bound for the true cost edges.
%     % Each edge in the graph can be described as a transition between configurations.
%     % Therefore, any edge that represents already computed time-optimal transition between its nodes configurations belongs to~$E_{\text{opt}}$.
%     % % Therefore, any edge that connects between nodes such that the true cost edge between their configurations was computed belongs to~$E_{\text{opt}}$.
%     % In~\tstar all the graph's edges are belonged to this set.

%     During the search, the algorithm maintains \textsc{Open} list for all the nodes that have been explored but not been expanded and \textsc{Closed} list for all expanded nodes. 
%     The final solution is configurations sequence of expanded nodes, which means that all of them are in the \textsc{Closed} list. 
%     Moreover, the sub-optimal solution includes configurations such that the transitions between them are time-optimal, their true cost were computed. 
%     % Thus, only nodes whose path from their parent to their configuration is time-optimal are expanded during the search algorithm.
%      Thus, only nodes whose the true cost of their transition already calculated are expanded during the search algorithm. 
%     % Thus, only nodes whose the edge to their predecessor is belonged to~$E_{\text{opt}}$ are expanded during the search algorithm. 
%     In each~\tstareps iteration, the algorithm uses a~\textsc{Focal} list to decide which node to expand. 
% \end{enumerate}

% \begin{equation}
% \footnotesize
%     \textsc{Focal} = \left\{ \text{n} \in \textsc{Open} \mid f(n) \leq (1+\varepsilon) \underset{\textup{n'}\in \textsc{Open}}{\min} f(\textup{n'}) \right\}.
%     \label{eq:focal}
% \end{equation}

% The proposed~\tstareps is summarized in Algorithm~\ref{alg:astareps-like}. The algorithm repeats until the \textsc{Open} list is empty (line 1), and in that case, there is no solution to the problem. The algorithm finds the next node to expand, denote as \text{next}(line 2), then removes it from the \textsc{Open} list and adds it to the \textsc{Closed} list (lines 3-4). 
% for each successor~$s$ of~$\textup{next.configuration}$, the cost of the path between them is calculated (line 6) and then the~$f$ cost of node~$s$ is calculated (line 7). When a new node is explored, it is necessary to determine if its configuration has already been explored, i.e. in the \textsc{Open} list, or has already been expanded, i.e. in the \textsc{Closed} list. 
% Accordingly, the algorithm determines if the path to the new node's configuration from the initial configuration~$s_{\text{start}}$ costs less than the previously explored node's configuration (referred to as~$n_{\textup{old}}$), reflected by the nodes'~$g$ costs. 
% If this is the case, the algorithm updates~$n_{\textup{old}}$ from the \textsc{Open} or \textsc{Closed} list and adds~$s$ to the \textsc{Open} list (lines 8-9). 
% \DP{For version with full description of~\astar (algorithm \ref{alg:astareps-like}).}

% The proposed~\tstareps is summarized in Algorithm~\ref{alg:astareps-like}. The algorithm repeats until the \textsc{Open} list is empty~(line 1), and in that case, there is no solution to the problem. The algorithm finds the next node to expand, denote as~\text{next}~(line 2), then removes it from the \textsc{Open} list and adds it to the \textsc{Closed} list~(lines 3-4).
% If the configuration of next is the goal configuration, the found sub-optimal path is returned~(line 5-6).
% for each successor~$s$ the configuration of next, the cost of the path between them is calculated~(line 8).
% A new node creates, denotes as~$n_{\textup{new}}$, and its~$g$ cost is calculated~(line 9).
% The algorithm determines if the configuration~$s$ already explored, i.e there is a node in \textsc{Open} that his configuration is~$s$~(line 10). 
% If such node is found, denote as~$n_{\textup{old}}$, the algorithm checks which node has lower~$g$ cost that indicates on a path with lest cost from~\start to~$s$~(lines 11-12).
% If the new node has a cheaper cost than the algorithm updates~$n_{\textup{old}}$~(line 13).

% If there is no node in \textsc{Open} such that its configuration is~$s$, it determines if there is such node in \textsc{Closed}~(line 16) and repeats the evaluation it did in lines 10-12.
% If the new node has chipper path cost from~\start to~$s$,~$n_{\textup{old}}$ is updated, it is removed from the \textsc{Closed} list, and added to the \textsc{Open} list~(lines 18-20).

% If the configuration~$s$ doesn't belong to any node either in \textsc{Open} and \textsc{Closed}, the algorithm calculates its fields to the new node and adds the node to the \textsc{Open} list~(lines 22-24).


% % When a new node is explored, it is necessary to determine if its configuration has already been explored, i.e. in the \textsc{Open} list, or has already been expanded, i.e. in the~\textsc{Closed} list. 

% \DP{For version without full description of~\astar.}

% \tstareps search step is based on~\astar search algorithm. Modifications we made to it involve deciding which node to expand at each iteration and the cost between predecessor and successor nodes. 

% \DP{Both version meet here.}
% % \tstareps aims to compute as few as possible time-optimal transitions.
% % % As mentioned above, in grid-based space there is a finite number of optional transitions.
% % When it expands a node and adds its neighbors as vertices to the graph, each edge can be defined by the transition between its nodes' configurations.
% % Those transitions can be time-optimal, and part of~$E_{\text{opt}}$, or lower bound to the time-optimal true cost.
% % Therefore, each node in the graph can be marked as having an edge between it and its parent time-optimal or not.
% % When it comes to finding the next node for expansion, it prefers nodes with edges from its' parent that belong to~$E_{\text{opt}}$, i.e. nodes that are the time-optimal from its parent state to its already calculated.
% % Thus, when it comes to find the next node for expansion it first looks for nodes that their~$f$ cost is not too grater than the~$f$ cost of the node at the top of the \textsc{Open} list, i.e part of \textsc{Focal}, and also that edge in the graph that connect them an their parent are belongs to~$E_{\text{opt}}$.

% % Algorithm~\ref{alg:find_next} summarizes the procedure for finding the next node to expand. %~(algorithm~\ref{alg:astareps-like} line 2). 
% % The algorithm looks for nodes that are in the~\textsc{Focal} list and the edge to their predecessor belongs to~$E_{\text{opt}}$~(line 1). 
% % After finding such a node, the algorithm returns the node with the lowest~$f$ cost that also meets the requirements~(line 2). 
% % If no such node is found, it computes the true cost of the edge between the node in the top of the \textsc{Open} list and its predecessor~(line 4).
% % After the algorithm computes the true cost for this edge,~$E_{\text{opt}}$ is updated. All the edges in the graph that represent the new computed time-optimal transition are added to~$E_{\text{opt}}$.
% % % After the algorithm computes the true cost for an edge that is evaluated by lower bound until this point, all the edges in the graph that represent the new computed time-optimal transition belong to~$E_{\text{opt}}$.
% % It repeats the procedure until the condition at line 1 is met~(line 6). 
% Algorithm~\ref{alg:find_next} summarizes the procedure for finding the next node to expand. %~(algorithm~\ref{alg:astareps-like} line 2).

% The algorithm checks whether there is any node in~$N_\text{opt}$ and returns the node with the lowest~$f$ cost in the set~(lines 1-2). If this set is empty, it computes the true cost of the transition of the node in the top of the \textsc{Open} list and its predecessor, denote as~$t_\textup{new}$~(line 3-5).
% After the algorithm computes the true cost for new it updates the true cost transitions~$T_\text{opt}$ set~(line 6). It repeats the procedure until the condition at line 1 is met~(line 7).

% % The algorithm looks for nodes that are both in the~\textsc{Focal} list and the true cost of their transition already computed~(line 1). 
% % After finding such a node, the algorithm returns the node with the lowest~$f$ cost that also meets the requirements~(line 2). 
% % If no such node is found, it computes the true cost of the transition of the node in the top of the \textsc{Open} list and its predecessor, denote as~$t_\textup{new}$~(line 3-5).
% % After the algorithm computes the true cost for new it updates the true cost transitions~$T_\text{opt}$ set~(line 6).
% % After the algorithm computes the true cost for this edge,~$E_{\text{opt}}$ is updated. All the edges in the graph that represent the new computed time-optimal transition are added to~$E_{\text{opt}}$.
% % After the algorithm computes the true cost for an edge that is evaluated by lower bound until this point, all the edges in the graph that represent the new computed time-optimal transition belong to~$E_{\text{opt}}$.
% % It repeats the procedure until the condition at line 1 is met~(line \ref{find-next_try_again}). 

% As mentioned above, in best-first-search algorithms each node~$n$ has~$g$ cost that represents the cost from~\start to~$n.\text{configuration}$. Specifically, the~$g$ cost consists of two components:~(i) the~$g$ cost of~$n.\text{parent}$ and~(ii) the path cost from~$n.\text{parent}$ to~$n.\text{configuration}$ . 

% Algorithm~\ref{alg:cost_func} summarizes~(ii) in~\tstareps. %~(algorithm~\ref{alg:astareps-like} line~6). 
% The algorithm determines whether the true cost of the edge that represents the transition between the configuration and its parent is already computed~(line 1). 
% If this is the case, the true cost of the transition~(line 2). 
% Otherwise, a lower bound for the true cost of it~(line 4). 
% The computational effort required for lower bound calculation is significantly less than that required by the time-optimal optimization for the transition between the same configurations.


% \begin{algorithm}[H]
% \SetAlgoLined
% \caption{\tstareps}
% \BlankLine
% %\KwIn{map,~$\mathbf{s}_\text{start}$,~$\mathbf{s}_\text{goal}$, \varepsilon, wind}
% \KwIn{$\text{map}, \mathbf{s}_\text{start}, \mathbf{s}_\text{goal}, \varepsilon, \text{wind}$}
% \KwOut{sub-optimal minimum-time path from~$\mathbf{s}_\text{start}$ to~$\mathbf{s}_\text{goal}$}
% \BlankLine
% Find the shortest path by using minimum speed Dubins paths\\
% Calculate time-optimal transitions for transitions that appeared at 1\\
%~\astareps-like search\\
% \end{algorithm}
% \newpage




% \begin{algorithm}[!t]
% %   \DontPrintSemicolon
%   \caption{\texttt{Find\_next\_node(\textsc{Open})}}
%   \label{alg:find_next}
% %   \BlankLine
%     \uIf{$\exists\, n \in \textsc{Focal} \land  e_\textup{n'}^\textup{n} \in E_{\textup{opt}}$}{
%              \KwRet~$\underset{n \in \textsc{Focal} \land  e_\textup{n'}^\textup{n} \in E_{\textup{opt}}}{\argmin} f(n)$}
% 	 \uElse{
% 	    compute true cost for the transition of~\text{OPEN.top() } \\
% 	    update~$E_{\textup{opt}}$ \\
% 	    \KwRet~$\text{next} \leftarrow \texttt{Find\_next\_node}(\texttt{OPEN})$}
% % }
% \end{algorithm}


% \begin{algorithm}[!t]
%   \caption{\texttt{cost(next.configuration,s)}}
%   \label{alg:cost_func}
% %   \DontPrintSemicolon
% %   \SetKwFunction{FMain}{cost}
% %   \SetKwProg{Fn}{Function}{:}{}
% %   \Fn{\FMain{successor, parent}}{
%     \uIf{$e(parent, configuration) \in E_{\textup{opt}}$}{
% 	         \KwRet true cost of~$e(parent, configuration)$}
% 	 \uElse{
% 	    \KwRet lower bound for the true cost of~$e(parent, configuration)$}
% % }
% \end{algorithm}
% \begin{algorithm}[!t]
% %   \DontPrintSemicolon
%   \caption{\texttt{find\_next\_node(\textsc{Open})}}
%   \label{alg:find-next_focal}
% %   \label{alg:find_next}
% %   \BlankLine
% % \While{true}{
%     \uIf{$\textsc{Focal} \neq \emptyset$}{ \label{find-next_check_focal}
%     % \uIf{$\exists\, n \in \textsc{Focal} \land  n.\textup{transition} \in T_{\textup{opt}}$}{
%      \KwRet~$\underset{n \in \textsc{Focal}}{\argmin} f(n)$} \label{find-next_return_argmin}
%     \uIf{$\textsc{Open} = \emptyset$}{ \label{find-next_open_empty} 
%         \KwRet \text{no solution} \label{find-next_go_out}
%     }
%   ~$n_\textup{top} \leftarrow \underset{n \in \textsc{Open}}{\argmin} f(n)$ \label{find-next_top_open} \\ 
%   ~$T_\text{new} \leftarrow n_\textup{top}.\text{T}$  \label{find-next_new_transition}\\
%     ~$ \mathcal{C}[T_\text{new}] \leftarrow c(T_\text{new})$ \label{find-next_compute_transition} \\
%     %~$ \mathcal{C} \leftarrow  \mathcal{C} \cup c(T_\text{new})$ \label{find-next_compute_transition} \\
%   ~$\kappa(T_{\textup{new}}) \leftarrow 1$ \label{find-next_update_kappa}\\
%   % update~$T_{\textup{opt}}$ \\
%     \KwRet~$\texttt{find\_next\_node(\textsc{Open})}$ \label{find-next_try_again} 
% % }
% \end{algorithm}


\ignore{
\begin{algorithm}[!t]
%   \DontPrintSemicolon
  \caption{\texttt{find\_next\_node(\textsc{Open})}}
  \label{alg:find-next_focal}
%   \label{alg:find_next}
%   \BlankLine
% \While{true}{
    \uIf{$\textsc{Focal} = \emptyset$}{ \label{find-next_focal_empty} 
        \KwRet \text{no solution} \label{find-next_go_out}
    }
   ~$n_\textup{focal} \leftarrow \underset{n \in \textsc{Focal}}{\argmin} f(n)$ \label{find-next_top_focal} \\
    \uIf{$\kappa(n_\textup{focal}.T) = 0$} { \label{find-next_check_focal_top}
        ~$\textsc{Focal}.\text{pop}()$ \label{find-next_pop_focal}\\
        \KwRet~$n_\textup{focal}$ \label{find-next_return_top}
    }
   ~$n_\textup{top} \leftarrow \underset{n \in \textsc{Open}}{\argmin} f(n)$ \label{find-next_top_open} \\ 
   ~$T_\text{new} \leftarrow n_\textup{top}.\text{T}$  \label{find-next_new_transition}\\
    ~$ \mathcal{C}[T_\text{new}] \leftarrow c(T_\text{new})$ \label{find-next_compute_transition} \\
    %~$ \mathcal{C} \leftarrow  \mathcal{C} \cup c(T_\text{new})$ \label{find-next_compute_transition} \\
   ~$\kappa(T_{\textup{new}}) \leftarrow 0$ \label{find-next_update_kappa}\\
   % update~$T_{\textup{opt}}$ \\
    \KwRet~$\texttt{find\_next\_node(\textsc{Open})}$ \label{find-next_try_again} 
% }
\end{algorithm}
}

% \begin{algorithm}[!t]
% %   \DontPrintSemicolon
%   \caption{\texttt{Find\_next\_node(\textsc{Open})}}
%   \label{alg:find_next}
% %   \BlankLine
%     \uIf{$N_\textup{opt} \neq \emptyset$}{
%     % \uIf{$\exists\, n \in \textsc{Focal} \land  n.\textup{transition} \in T_{\textup{opt}}$}{
%      \KwRet~$\underset{n \in N_\textup{opt}}{\argmin} f(n)$}
%    ~$n_\textup{top} \leftarrow \underset{n \in \textsc{Open}}{\argmin} f(n)$\\
%    ~$t_\text{new} \leftarrow n_\textup{top}.\text{transition}$\\
%    ~$\textup{compute true cost of } t_\text{new}$ \\
%    ~$T_{\textup{opt}} \leftarrow T_{\textup{opt}} \cup t_{\textup{new}}$\\
%   % update~$T_{\textup{opt}}$ \\
%     \KwRet~$\text{next} \leftarrow \texttt{Find\_next\_node}(\textsc{Open})$
% % }
% \end{algorithm}

% \begin{algorithm}[!t]
%   \caption{\texttt{cost(s}\texttt{,g)}}
%   \label{alg:cost_func-kappa}
% %   \DontPrintSemicolon
% %   \SetKwFunction{FMain}{cost}
% %   \SetKwProg{Fn}{Function}{:}{}
% %   \Fn{\FMain{successor, parent}}{
% 	 \uIf{$\kappa(T_{\text{s}}^\text{g})=1$}{ \label{cost_func-k_value}
% 	         \KwRet~$\mathcal{C}[T_\textup{s}^\textup{g}]$} \label{cost_func-true_cost}
% 	 \uElse{
% 	    \KwRet~$\hat{c}(T_\textup{s}^\textup{g})$} \label{cost_func-lower_bound}
% % }
% \end{algorithm}


% \begin{algorithm}[!t]
%   \caption{\texttt{cost(next.configuration,s)}}
%   \label{alg:cost_func-kappa}
% %   \DontPrintSemicolon
% %   \SetKwFunction{FMain}{cost}
% %   \SetKwProg{Fn}{Function}{:}{}
% %   \Fn{\FMain{successor, parent}}{
% 	 \uIf{$\mathcal{T}_\textup{next.configuration}^\textup{s} \in T_{\textup{opt}}$}{
% 	         \KwRet true cost from \text{next.configuration} to s}
% 	 \uElse{
% 	    \KwRet lower bound for the true cost from \text{next.configuration} to s}
% % }
% \end{algorithm}

% As with~\cite{Wolek} and the library they published,~\tstar original work did not include wind. It was necessary to modify the library to include wind conditions in the optimization constraints for the algorithm to consider those conditions fully.

% \section{Computing lower bound}
%~\tstareps finds a sub-optimal solution with a significant reduction of the runtime. 
% The algorithm saves time due to a decrease in the total number of time-optimal transition optimizations that have to be calculated during the running of the algorithm. Time is reduced by using the lower bound for edges whose time-optimal transition has not yet been calculated. 

% Calculating the lower bound takes only a fraction of the time of time-optimal optimization for the same transition. The lower bound has to be both optimistic, i.e its cost will be smaller than the real cost, and as informative, i.e its cost should be \textsc{Closed} to the real cost, as it can. 
% The closer the lower bound is to the time-optimal transition, the fewer total calculated time-optimal transitions will exist. 

% In this work, two lower bound options for the algorithm were examined.
% The lower bound for the turning radius is determined based on the wind speed. 
% Let assume, w.l.o.g, that the wind direction is parallel to the 
% x-axis, and thus~$w_y = 0$. 
% Then the wind can be easily described by its relative speed to the airspeed of the vehicle~$v$
% \begin{equation}
% w_x = \alpha\, v %,  \: \: 0 \leq \alpha < 1
% \end{equation}

% The lower bound radius~(in the reference frame of the ground) is determined based on the minimum turning radius~$\rho _[\min}$
% \begin{equation}
%     \rho_\text{LB} = (1-\alpha) \, \rho _[\min}
%     \label{r_min_wind}
% \end{equation}{}

% The first option of the lower bound assumes that the vehicle can travel at maximum-speed and turn with the minimum turning radius between consecutive configurations:
% \begin{equation}
%     LB_1 = \frac{\text{Dubins paths}(\rho_\text{LB})}{v _{\max} + \vert \vec{w} \vert}
%     \label{LB1}
% \end{equation}
% Where \text{Dubins paths}($\rho$) denotes the Dubins paths between two configurations using turning radius~$\rho$.

% The second option of lower bound is to use the ground speed which is based on the direction of the transition between the consecutive configurations:
% \begin{equation}
%     s_{i_\text{position}} = s_i (\hat{x} + \hat{y})^T
% \end{equation}

% \begin{equation}
%     \hat{s} = \frac{s_{2_\text{position}} - s_{1_\text{position}}}{\vert s_{2_\text{position}} - s_{1_\text{position}} \vert}
% \end{equation}

% \begin{equation}
%     v_{\textup{ground}} = \hat{s} \cdot \vec{w} + \sqrt{(\hat{s} \cdot \vec{w})^2 + v _{\max}^2 -\vert \vec{w} \vert ^2 }
% \end{equation}

% \begin{equation}
%     LB_2 = \frac{\text{Dubins paths}(\rho_\text{LB})}{v_{\textup{ground}}}
%     \label{LB2}
% \end{equation}
% Fig.~\ref{fig:lower_bound} shows a comparison between the options of lower bound for the time-optimal transitions when higher is better since it leads to tighter lower bound and to better estimation of the actual cost of the time-optimal transition. As can be seen, the lower bound that uses ground speed is more informative than the version that assumes the vehicle can travel at maximum speed and turn with the smallest radius.
% \begin{figure}[!t]
%     \centering
%     % \adjustbox{margin=1em,width=\textwidth,set height=4cm,set depth=4cm,frame,center}{\includegraphics[scale=0.6]{pics/Lower bound quality}}
%     \includesvg[scale=0.5]{pics/Lower bound quality for paper.svg}
%     % {\includegraphics[scale=0.6]{pics/Lower bound quality}}
%     \caption{Average of the ratio between the lower bound and time-optimal costs vs. wind's modulus.}
%     \label{fig:lower_bound}
% \end{figure}


% % https://www.wolframalpha.com/input/?i=integrate+1+%2F+%28a+*+cos%28x%29+%2B+sqrt%281+-+a%5E2+*+%28sin%28x%29%29%5E2%29%29+dx

% This leads to the elliptic integral!

% Implemented in SpecialFunctions.jl
% \url{https://github.com/JuliaMath/SpecialFunctions.jl}

% \begin{figure}[!b]
%     \centering
%     % \adjustbox{margin=1em,width=\textwidth,set height=4cm,set depth=4cm,frame,center}{\includegraphics[scale=0.6]{pics/Lower bound quality}}
%     \includesvg[scale=0.5]{pics/Lower bound quality for paper with fill.svg}
%     % {\includegraphics[scale=0.6]{pics/Lower bound quality}}
%     \caption{Average of the ratio between the lower bound and time-optimal costs vs. wind's modulus.}
%     \label{fig:lower_bound_wind}
% \end{figure}



% \begin{figure*}[h]
%     \centering
%     \begin{subfigure}{.45\textwidth}
%         \includesvg[width=1\linewidth]{pics/Number of total transitions.svg}
%         % {\includegraphics[scale=0.6]{pics/Lower bound quality}}
%         \caption{}
%     \end{subfigure}
%     \begin{subfigure}{.4\textwidth}
%         \includesvg[width=1\linewidth]{pics/eps_1_5_winx_02_windy_01.svg}
%         % {\includegraphics[scale=0.6]{pics/Lower bound quality}}
%         \caption{}
%     \end{subfigure}
%     \caption{Total number of time-optimal transitions that were calculated during the algorithm, comparison with and without use the shortest path as a heuristic~(a) and Path of~\tstareps solution for~$\varepsilon=1.5$ with wind condition of~$\vec{w}=0.2\hat{x}+0.1\hat{y}$(b).}
%     \label{fig:total transitions}
% \end{figure*}

% - tstarepsion-alg.tex -------------------------------------------------------

%$n \leftarrow \texttt{find\_next\_node(\textsc{Open})}$ \label{tstareps-find_next}\\
%~~~~\DP{\textbf{continue to next iteration}} \\
% ~$\text{Succ(}n\text{)} \leftarrow \forall n', n'.\text{parent}=n$\\


% - results.tex ---------------------------------------------------------------

\ignore{
We demonstrate how computing initial sub-set of time-optimal transitions, and especially the set who appears in the shortest path solution, the number of computed transitions in~\tstareps can reduces.

In this scenario, we examined the number of computed time-optimal transitions in~\tstareps with and without first finding the shortest path from the initial configuration~$s_{\text{start}}$ to the goal configuration~$s_{\text{goal}}$ as described at~\ref{sec:tstareps}. 
Specifically, we tested whether using shortest and time-optimal paths connection reduced the number of computed transitions and, therefore, the runtime of~\tstareps.

This instance can be seen in Fig.~\ref{fig:wind_results_0_2_x-a} except the presented examination was during no wind conditions.
   
Fig.~\ref{fig:total_transitions} shows that the number of time-optimal transitions as a function of the~$\varepsilon$ is a monotonically decreasing function. 
The total number of computed time-optimal transitions and therefore the runtime of the algorithm is reduced using the shortest path from~\start to~\goal compared to finding a sub-optimal solution without the aid of the shortest path. 
}

% \begin{figure}[tb]
%     \centering
%     \begin{subfigure}{.23\textwidth}
%         \includesvg[width=1\linewidth]{pics/map_18_num_of_time_optimal_various_lower_bound.svg}
%         \caption{}
%         \label{fig:lower_bound_no_wind-a}
%     \end{subfigure}
%     %\hfill
%     \begin{subfigure}{.23\textwidth}
%         \includesvg[width=1\linewidth]{pics/map_18_time_duration_various_lower_bound.svg}
%         \caption{}
%         \label{fig:lower_bound_no_wind-b}
%     \end{subfigure}
%     \caption{
%     Comparing the effect of different lower bounds.
%     \protect
%     (\subref{fig:lower_bound_no_wind-a})~Total number of time-optimal transitions calculated 
%     and
%     (\subref{fig:lower_bound_no_wind-b})~computation time of~\tstareps, respectively,
%     for each lower bound and for several values of~\eps. 
%     }
%     \label{fig:lower_bound_no_wind}
% \end{figure}

% {\includegraphics[scale=0.6]{pics/Lower bound quality}}
% \vspace{2mm}

% {\includegraphics[scale=0.6]{pics/Lower bound quality}}
% \vspace{-1mm}

% {\includegraphics[scale=0.6]{pics/Lower bound quality}}

%Following the previous lower bound analysis, the lower bound for true cost was Dubins path using turning radius~$\rho _{\min}$ without consideration for obstacles divided by the maximum speed~$v _{\max}$.
%It is assumed in this scenario that prepossessing all time-optimal transitions for~\tstar can be computed offline, and its duration can thus be ignored at runtime. 

%The results are summarised in Fig.~\ref{fig:no_wind_results}. 
%Fig.~\ref{fig:no_wind_results-a} shows the found sub-optimal path by~\tstareps for~$\varepsilon=3$.
%The most computationally expensive component in the~\tstareps algorithm is the time-optimal optimizations~\ref{fig:no_wind_results-b}.
%Notice that the total runtime of the algorithm reduces with~\eps~\ref{fig:no_wind_results-c}.
%However, if~\tstar can calculate all the time-optimal transitions offline its runtime is significantly smaller than any choice of~\eps in~\tstareps.

% \vspace{0mm} 
% \vspace{1mm}

% {\includegraphics[scale=0.6]{pics/Lower bound quality}}

% \vspace{2mm}
% {\includegraphics[scale=0.6]{pics/Lower bound quality}}

% {\includegraphics[scale=0.6]{pics/Lower bound quality}}

% {\includegraphics[scale=0.6]{pics/Lower bound quality}}
% {\includegraphics[scale=0.6]{pics/Lower bound quality}}

% \DP{
   % \subsection{Additional suboptimal motion-planning algorithms}
   % Considering works that aim to find a suboptimal solution for minimum-time curvature-constrained systems, how their performance compares with this work, and what guarantees each provides, is worth mentioning.
   % As mentioned, Wilson et al.~\cite{GMDM} reduced computational effort by allowing the system to travel with Dubins motions but in several radii, and evaluated this approach for three.
   % Their model does not have guarantees for the solution quality considering the system can travel at variable speeds.
   % From a comparison with our implementation of their algorithm in several instances, we found that their algorithm's last order of magnitude less than \tstareps but with an average higher cost of~$18\%$.
   % On the other hand, in a dynamic environment, their approach has both no guarantees of the solution quality and computational efficacy reduces and possibly goes since, in this setting, Dubins path has no analytical solution and needs to be computed by solving a root-finding problem which is computationally expensive~\cite{minimum_time_const_wind}.
   % A method of tackling the problem of fast computation for Dubins maneuvers in a dynamic environment has been developed by~\cite{Dubins_with_currents}.
   % A fast solution is found by using only two of the Dubins types, those with an analytical solution.
   % However, this approach both uses only two types of Dubins so there are no guarantees, and also allows the vehicle to perform larger turn segments up to~$4\pi$ so the solution cost is affected accordingly.
   % }

\ignore{
      \DP{
	 \subsection{Additional suboptimal motion-planning algorithms}
	 \label{subsec:additional_approaches}
	 Several works, which also were reviewed in~\ref{sec:related_work}, wish to overcome the same challenge as this work, i.e reduce computational effort by relaxing the optimality of curvature-constrained motion planner.
	 In this section, we will briefly compare their performance and show why the comparison to~\tstar is the most appropriate for this work.
	 }

	 \DP{
	    Wilson et al.~\cite{GMDM} reduced computational effort by allowing the system to travel with Dubins motions but in several radii, and evaluated this approach for three different radii.
	    Their model intends to reduce the runtime and with no great compromise on its solution cost, but with no guarantees regarding the quality.
	    From our comparison between~\tstareps and Wilson's model we found that in static conditions, Wilson's lasts an order of magnitude less than~\tstareps and with greater cost by average of \SI{18}{\percent}.
	    However, in windy conditions, their approach has both no guarantees of the solution quality and computational efficacy reduces and potentially fade. In this setting, Dubins path has no analytical solution and needs to be computed by solving a root-finding problem which is computationally expensive~\cite{minimum_time_const_wind}.
	    }

	    \DP{
	       A method to tackle the problem of fast computation for Dubins maneuvers in a dynamic environment, has been developed by~\cite{Dubins_with_currents}.
	       However, this method's main objective is to perform online motion-planning under ocean currents. 
	       The cost of the computed solution has minor importance. 
	       For the same transition that was shown in their work, using our modified model that considers wind and is publically available, a time cost of~$3.88$~sec was achieved when~\cite{Dubins_with_currents} achieved~$10.51$~sec.
	       }

	       \DP{
		  Thus, in our opinion and follow the mention above,~\tstar is the most suitable algorithm for comparison with~\tstareps.
		  }

		  }

\ignore{
   We will compare~\tstareps and~\tstar under windy conditions.
   Since the wind potentially can be in any direction and any force, to assure that the found path by~\tstar will be collision-free, it can not computes the time-optimal transitions offline and has to do so during the running of the algorithm.
   When~\tstareps computes time-optimal transition on demand,~\tstar must calculate all the optional transitions and cache them in a table. 
   During the search for a path from~\start to~\goal,~\tstar creates a query to this table to get the time-optimal transitions between connective configurations.
   contrary to static environmental conditions, in the general case of windy conditions rotation and symmetry between transitions can not be considered the same. 
   Thus, in these conditions, the total number of time-optimal transitions is~512.

   In these environmental conditions, the dynamic model of the system, the lower bound of the transitions' true cost, and the constraints of the time-optimal optimization have to be modified to consider wind. Those modifications are described in detail in the appendix.

   % Furthermore, as shown in Fig.~\ref{fig:lower_bound_wind}, the lower bound become less tight with the wind modulus so we assumed that this scenario would be challenging for~\tstareps.

   The results are summarised in Fig.~\ref{fig:wind_results_0_4_x_0_1_y}.
   Fig.~\ref{fig:wind_results_0_4_x_0_1_y-a}. shows the found sub-optimal path by~\tstareps for~$\varepsilon=0.5$.
   The most computationally expensive component in both~\tstareps and~\tstar is still the time-optimal optimizations and it lasts two orders of magnitude more than any other algorithm step Fig.~\ref{fig:wind_results_0_4_x_0_1_y-b}. 
   Notice that for any value of~\eps,~\tstareps reduces the runtime compared to~\tstar.
   This reduction grows with~\eps and can save a significant amount of computational time and can accelerate the runtime by a factor of~$57\times$ Fig.~\ref{fig:wind_results_0_4_x_0_1_y-c}.
}

% In addition, the cost for all~\eps values is in the range of~$1+\varepsilon$ the optimal~\ref{fig:wind_results_0_4_x_0_1_y}~(c).
% Notice that the total runtime of the algorithm reduces with~\eps~\ref{fig:wind_results_0_4_x_0_1_y}~(c).
% However, if~\tstar can calculate all the time-optimal transitions offline its runtime is significantly smaller than any choose of~\eps in~\tstareps.


% We evaluate~\tstareps empirically in two environmental conditions in this section.
% Several options for true edge cost lower bound was examined.
% In addition, the approach of finding the shortest path from~$s_{\text{start}}$ to~$s_{\text{goal}}$ at the beginning of the algorithm will be validated by comparing it to the algorithm without the shortest path search.
% % First, we evaluate performance of~\tstareps and our implementation of~\tstar in static environmental conditions. 
% % The algorithms performance will also be evaluated in a scenario involving windy conditions in space. 
% % Both scenarios will be evaluated for several values of \eps, the sub-optimal parameter.

% % Each cell in the instances' grids was either labeled as an open space or an obstacle as described in section~\ref{sec:problem}. 
% All experiments were run on a 3.1GHz Intel Core i9 processor with 32GB of memory.


% We consider the following kinematics parameters for the robotic-system: the maximum and minimum velocities are~$v _{\max} = 1 \, \text{m/s}$,~$v _{\min}=0.5\, \text{m/s}$. 
% The speed of the wind must be smaller than the minimum speed~$\vert \vec{w} \vert \leq v _{\min}$. 
% The turning rate set to~$u _{\max} = 1\, \text{rad/s}$. The radii are functions of the vehicle speed, the turning rate, the wind~(both direction and force) and the heading angle~$\rho = \frac{f(v,\vec{w},\theta)}{u _{\max}}$. 
% Also, this work considers 8 optional orientations in each configuration and 8 neighbors for each cell in the grid. 

% The search area consists of~$15 \times 15$ cells.~$s_{\text{start}} = (1,1,0,0.5)$ and~$s_{\text{goal}}=(2,12,\frac{\pi}{2},0.5)$. Each cell in the grid was either labeled as an open space or an obstacle as described at section~\ref{sec:problem}. All experiments were run on a 3.1GHz Intel Core i9 processor with 32GB of memory.


% \begin{figure*}[h]
%     \centering
%     \begin{subfigure}{.45\textwidth}
%         \includesvg[width=1\linewidth]{pics/map6_windx_0_2_runtime_vs_cost.svg}
%         % {\includegraphics[scale=0.6]{pics/Lower bound quality}}
%         \caption{}
%     \end{subfigure}
%     \begin{subfigure}{.45\textwidth}
%         \includesvg[width=1\linewidth]{pics/map6_windx_0_2_time_duration.svg}
%         % {\includegraphics[scale=0.6]{pics/Lower bound quality}}
%         \caption{}
%     \end{subfigure}
%     \caption{Runtime vs. cost for~\tstar and~\tstareps with various values of \eps~(a) and time duration in seconds for each component in the algorithms~(b).}
%     \label{fig:tstar_vs_epsilon}
% \end{figure*}
% \begin{enumerate}[A.]
%     \item \textit{\tstareps with and without finding the shortest path at the beginning of the algorithm} \\
% %   Since the most computationally expensive part of the algorithm is the time-optimal optimizations, it aims to do so as few as possible. 
%     We demonstrate how computing initial sub-set of time-optimal transitions, and especially the set who appears in the shortest path solution, the number of computed transitions in~\tstareps can reduces.

%   In this scenario, we examined the number of computed time-optimal transitions in~\tstareps with and without first finding the shortest path from the initial configuration~$s_{\text{start}}$ to the goal configuration~$s_{\text{goal}}$ as described at~\ref{sec:tstareps}. 
%   Specifically, we tested whether using shortest and time-optimal paths connection reduced the number of computed transitions and, therefore, the runtime of~\tstareps.
% %   Each initial configuration can have one of eight optional heading angles, and each of its eight neighbors can also have one of those eight options. 
% %   Thus, the maximum number of time-optimal transitions is 512. 

% %   The presented examination was during wind conditions of~$\vec{w}=0.2\hat{x}+0.1\hat{y}$ in the map showed in Fig.~\ref{fig:wind_results_0_2_x}(a). 
%   The search area consists of~$15\times15$ cells where each cell was marked as free or occupied by an obstacle. Robotic-system parameters was~$v _{\min}= 0.5\,\textup{m/s}$ and~$u _{\max}=1\,\textup{rad/s}$.
%   The initial and goal configurations as follow:~$s_{\text{start}}=(1,1,0,0.5)$ and~$s_{\text{goal}}= (12,2,\frac{3\pi}{2},0.5)$.
%   This instance can be seen in Fig.~\ref{fig:wind_results_0_2_x}~(a) except the presented examination was during no wind conditions.

%   Fig.~\ref{fig:total_transitions} shows that the number of time-optimal transitions as a function of the~$\varepsilon$ is a monotonically decreasing function. 
%   The total number of computed time-optimal transitions and therefore the runtime of the algorithm is reduced using the shortest path from~\start to~\goal~(dashed blue line) compared to finding a sub-optimal solution without the aid of the shortest path~(purple line). 
% %   The dashed yellow line shows the number of transitions that appeared in the shortest path, and this number is the minimum number of the time-optimal calculated transitions when using the shortest path as a heuristic for the initial set of time-optimal transitions.
%     The dashed yellow line shows the number of transitions that appeared in the shortest path, and this number represents the number of time-optimal transitions in the initial set of time-optimal transitions.

%   \item \textit{Edge true cost lower bound}\\
%   As described in~\ref{sec:tstareps}, there are many options to choose lower bound for the true cost of time-optimal transition.
%   As the lower bound being informative, its cost being close to the real cost, the number of computed time-optimal transitions during the algorithm will reduce.
%   A lower bound should also be easy to calculate because its main purpose is to save the computational time. % of expensive time-optimal transitions computations.
%   In this work, three options of lower bound were examined:
%   \begin{enumerate}
%       \item Euclidean distance which is easy to calculate but in the case of curvature-constrained, not very informative.
%       \item minimum speed Dubins path with consideration for obstacles which is very informative but not necessarily computationally cheap to evaluate.
%       \item minimum speed Dubins path without consideration for obstacles which is not as informative as the version with awareness to the obstacles but should be cheaper to calculate.
%   \end{enumerate}
%   In order to ensure the lower bounds are optimistic, their cost smaller that the true cost, each of them is divided by~$v _{\max}$.
%   The search area consists of~$30\times30$ cells. 
%   Robotic-system parameters was~$v _{\min}=0.6\,\textup{m/s}$ and~$u _{\max}=0.75\,\textup{rad/s}$.
%   The initial and goal configurations as follow:~$s_{\text{start}}=(28,28,\pi,0.5)$ and~$s_{\text{goal}}=(1,1,\frac{3\pi}{2},0.5)$.
%   The scenario map can be seen in~\ref{fig:wind_results_0_4_x_0_1_y}~(a).

%   Fig.~\ref{fig:lower_bound_no_wind} summarizes the comparison between those lower bound options.
%   It can be seen that Euclidean distance lower bound performers poor results, the total number of time-optimal transitions and hence runtime, because of its lack of information it provides.
%   The Dubins path with obstacles awareness lower bound provides the best results consider the number of computed time-optimal transitions~\tstareps has to do.
%   However, its evaluation is relatively expensive and it is reflected in the total runtime of~\tstareps.
%   Even in cases where less time-optimal transitions were computed, the duration of~\tstareps that uses a lower bound that considers obstacles lasted longer than the version that does not consider them.
%   A Dubins path without considering obstacles lower bound balances well between informative and computational effort.

% \item \textit{Static environmental conditions}\\
% We will compare~\tstareps and~\tstar in scenario where there are no dynamic environmental conditions such as wind or ocean currents.
% Following the previous lower bound analysis, the lower bound for true cost was Dubins path using turning radius~$\rho _{\min}$ without consideration for obstacles divided by the maximum speed~$v _{\max}$.
% % In this case, the lower bound for non-time-optimal transitions as described in algorithm~\ref{alg:cost_func} is Dubins path using turning radius~$\rho _{\min}$ divided by the maximum speed~$v _{\max}$.
% The search area consists of~$15\times15$ cells. 
% Robotic-system parameters was~$v _{\min}=0.6\,\textup{m/s}$ and~$u _{\max} = 0.9\,\textup{rad/s}$.
% The initial and goal configurations as follow:~$s_{\text{start}}= (1,2,0,0.5)$ and~$s_{\text{goal}} = (1,9,\frac{3\pi}{2},0.5)$.
% It is assumed in this scenario that prepossessing all time-optimal transitions for~\tstar can be computed offline, and its duration can thus be ignored at runtime. 

% The results are summarised in Fig.~\ref{fig:no_wind_results}. 
% Fig.~\ref{fig:no_wind_results}~(a) shows the found sub-optimal path by~\tstareps for~$\varepsilon=3$.
% The most computationally expensive component in the~\tstareps algorithm is the time-optimal optimizations~\ref{fig:no_wind_results}~(b).
% Notice that the total runtime of the algorithm reduces with~\eps~\ref{fig:no_wind_results}~(c).
% However, if~\tstar can calculate all the time-optimal transitions offline its runtime is significantly smaller than any choice of~\eps in~\tstareps.

% \item \textit{Dynamic environmental conditions}\\
% We will compare~\tstareps and~\tstar under windy conditions.
% Since the wind potentially can be in any direction and any force, to assure that the found path by~\tstar will be collision-free, it can not computes the time-optimal transitions offline and has to do so during the running of the algorithm.
% When~\tstareps computes time-optimal transition on demand,~\tstar must calculate all the optional transitions and store them in a table. 
% During the search for a path from~\start to~\goal,~\tstar creates a query to this table to get the time-optimal transitions between connective configurations.
% contrary to static environmental conditions, in the general case of windy conditions rotation and symmetry between transitions can not be considered the same. 
% Thus, in these conditions, the total number of time-optimal transitions is~512.

% In these environmental conditions, the dynamic model of the system, the lower bound of the transitions' true cost, and the constraints of the time-optimal optimization have to be modified to consider wind. Those modifications are described in detail in the appendix.

\ignore{
   \begin{figure*}[h]
      \centering
      \begin{subfigure}[b]{.225\textwidth}
	 \includesvg[width=1\linewidth]{pics/map18_eps_1_5_windx_04_windy_01_2.svg}
	 \caption{}
	 \label{fig:wind_results_0_4_x_0_1_y-a}
	 \vspace{2mm}
      \end{subfigure}
      \begin{subfigure}[b]{.315\textwidth}
	 \includesvg[width=1\linewidth]{pics/map18_windx_0_4_windy_0_1_time_duration.svg}
	 \caption{}
	 \label{fig:wind_results_0_4_x_0_1_y-b}
	 \vspace{2mm}
      \end{subfigure}
      \begin{subfigure}[b]{.335\textwidth}
	 \includesvg[width=1\linewidth]{pics/map18_windx_0_4_windy_0_1_runtime_vs_cost.svg}
	 \caption{}
	 \label{fig:wind_results_0_4_x_0_1_y-c}
      \end{subfigure}
      \caption{~\tstareps solution for~$\varepsilon=0.5$ 
      \protect
      (\subref{fig:wind_results_0_4_x_0_1_y-a}), the blue arrows represent the wind condition vector. Time duration in seconds for each component in the algorithms 
      \protect
      (\subref{fig:wind_results_0_4_x_0_1_y-b}) and runtime vs. cost in seconds for~\tstar and~\tstareps for several \eps values 
      \protect(\subref{fig:wind_results_0_4_x_0_1_y-c}).}
      \label{fig:wind_results_0_4_x_0_1_y}
   \end{figure*}
   }



% The search area consists of~$30\times30$ cells. 
% Robotic-system parameters was~$v _{\min}=0.5\,\textup{m/s}$ and~$u _{\max}= 1\,\textup{rad/s}$.
% The initial and goal configurations as follow:~$s_{\text{start}} =(28,28,\pi,0.5)$ and~$s_{\text{goal}}= (1,1,\frac{3\pi}{2},0.5)$.
% The wind conditions was~$\vec{w}=0.4\hat{x}+0.1\hat{y}$. 
% These wind conditions are close to the possible maximum since they have to be smaller than the minimum speed~$v _{\min}$ so we assumed that this scenario would be challenging for~\tstareps.
% \footnote{\DP{Consider to remove the last sentance.}}
% % Furthermore, as shown in Fig.~\ref{fig:lower_bound_wind}, the lower bound become less tight with the wind modulus so we assumed that this scenario would be challenging for~\tstareps.

% The results are summarised in Fig.~\ref{fig:wind_results_0_4_x_0_1_y}.
% Fig.~\ref{fig:wind_results_0_4_x_0_1_y}~(a) shows the found sub-optimal path by~\tstareps for~$\varepsilon=0.5$.
% The most computationally expensive component in both~\tstareps and~\tstar is still the time-optimal optimizations and it lasts two orders of magnitude more than any other algorithm step. 
% % It can be seen that the duration of adding the shortest path finding in~\tstareps is negligible~\ref{fig:wind_results_0_4_x_0_1_y}~(b).
% Notice that for any value of~\eps,~\tstareps reduces the runtime compared to~\tstar.
% This reduction grows with~\eps and can save a significant amount of computational time~\ref{fig:wind_results_0_4_x_0_1_y}~(c).
% % In addition, the cost for all~\eps values is in the range of~$1+\varepsilon$ the optimal~\ref{fig:wind_results_0_4_x_0_1_y}~(c).
% % Notice that the total runtime of the algorithm reduces with~\eps~\ref{fig:wind_results_0_4_x_0_1_y}~(c).
% % However, if~\tstar can calculate all the time-optimal transitions offline its runtime is significantly smaller than any choose of~\eps in~\tstareps.

% \end{enumerate}


% \begin{enumerate}[A.]
%     \item \textit{\tstareps with and without finding the shortest path at the beginning of the algorithm} \\
%   Since the most computationally expensive part of the algorithm is the time-optimal optimizations, we want to do so as few as possible. 

%   In this scenario, we examine the number of total time-optimal optimizations in the algorithm with and without first finding the shortest path from the initial configuration~$s_{\text{start}}$ to the goal configuration~$s_{\text{goal}}$. 
%   In this comparison, we test whether the use of the connection between the shortest and time-optimal paths reduces the runtime of the algorithm. 
%   Each initial configuration can have one of 8 optional heading angles, and each of its 8 neighbors can also have one of those 8 options. 
%   Thus, the maximum number of time-optimal transitions is 512. 

%   The presented examination was during wind conditions of~$\vec{w}=0.2\hat{x}+0.1\hat{y}$. 

%   Notice that the number of time-optimal transitions as a function of the~$\varepsilon$ is a monotonically decreasing function~(Fig.~\ref{fig:total transitions}a), the blue arrows show the wind vector. 
%   Also, the number of total time-optimal calculated transitions and therefore the total runtime of the algorithm is reduced using the shortest path from~\start to~\goal~(blue line) compared to finding a sub-optimal solution without the aid of the shortest path~(purple line). 
%   The dashed yellow line shows the number of transitions that appeared in the shortest path, and this number is a lower bound to the number of the time-optimal calculated transitions. 
%   Fig.~\ref{fig:total transitions}b shows a sub-optimal solution for~$\varepsilon=1.5$.

%     \item \textit{Comparison between~\tstareps and~\tstar involving windy conditions} \\
%     Now, we will examine the performance of~\tstareps compared to~\tstar and show how using the shortest path as an initial guess of which of the transitions between configurations have a high probability to be part of the solution sequence and that way save computational time. 

%     We choose to examine our algorithm in a dynamic environment that involves wind, and we will show that in these conditions, the optimal solution lasts much longer than the sub-optimal that is found by~\tstareps. 
%     In dynamic environmental conditions, all the optional transitions can not be calculated offline and have to be calculated during the algorithm running. 
%     When~\tstareps calculates time-optimal transition on demand,~\tstar must calculate all the optional transitions and store them in a table. 

%     During the search for a path from~\start{} to \goal,~\tstar creates a query to the table to get the time-optimal transitions between connective configurations. 
%     The presented examination was during wind conditions of~$\vec{w}=0.2\hat{x}$. 

%     Fig.~\ref{fig:tstar_vs_epsilon}a shows a comparison between the runtime of the algorithms and the path cost of the found solutions. It can be seen that~\tstareps reduces the runtime and the cost is confirmed by the defined upper-bound. In addition, the figure demonstrates how the runtime decreases with \eps as a result of fewer time-optimal transitions that have been calculated. Fig~\ref{fig:tstar_vs_epsilon}b shows the duration of each component of the main three components as defined in~\ref{sec:tstareps}. Time-optimal optimizations remain the most computationally expensive portion of the algorithm, with a cost of more than~$99\%$ of the runtime. The adding of the shortest path finding at the beginning of the algorithm is negligible compare to the total runtime. The search part of~\tstareps lasts a bit longer than the~\tstar search, in absolute time. It occurs because of the procedure of finding the next node for expansion that takes more time than just expand the node at the top of the \textsc{Open} list as in~\tstar.
% \end{enumerate}

% - conclusion.tex ------------------------------------------------------------

% Time-optimal transitions can be calculated at the beginning of the algorithm and produce better results than incrementally calculating when needed.
% However, even though there are only a few unique time-optimal transitions, a significantly greater number of time-optimal transitions are calculated when the wind is close to the possible high or where~$\varepsilon$ close to~0. 
   % The next step would be to find a minimal set of time-optimal transitions that include all transitions needed for the optimal solution. 
   % Test~\tstareps in continuous space problems and use the technique for reducing the number of collision detection for edges in the graph, the action that determines whether an edge in the graph is collision-free.
   % This action is one of the most computationally expensive parts in motion-planning in continuous space and compares the performance to other algorithms that claim to do so such as~\cite{lbt-rrt}.
   %

   % \DP{
% In this work we presented~\tstareps, a novel algorithmic framework for finding bounded-suboptimal solution of a motion-planning problem.
% We presented how by reducing the most computationally expensive component the runtime can be reduced significantly.
% Our key contribution is the diagnosis that a major portion of the robotic-system's transition between configurations is not used as part of the solution for the motion-planning problem.
% This diagnosis becomes extremely useful in discrete space where there is a finite number of transitions and those that have already been computed can reuse.
% }

\ignore{
\DP{
Currently,~\tstareps reduces the number of transitions computation but yet computes more transitions than it uses in the found path, especially when~\eps value is close to~$0$.
It may be possible to develop a lower bound that is more informative to guarantee a reduction of the total number of computed transitions.
Another future work can utilize the fact that even after reducing the number of computed transitions, it is still the most computationally expansive component of~\tstareps, and the search part lasts a negligible portion of it.
Therefore, following the work in~\cite{any_time_astar},~\tstareps can become a version of \emph{anytime}~\astar.
For any set of computed transitions, the algorithm searches for a solution path whose cost decreases with incrementally computed transitions.
}}

%~\tstareps algorithm suggests a novel approach that uses the connection between the shortest and time-optimal paths to find a solution in a short amount of time and with an upper-bound of its cost.
% The search algorithm we use is based on~\astar algorithm and specifically inspired by~\astareps~\cite{astareps}. This connection is reflected in the fact that the shortest and time-optimal path usually share the same homotopy class. The algorithm has 3 main parts:~(i) First, it finds the shortest path from~$s_{\text{start}}$ to~$s_{\text{goal}}$ by using Dubins paths at minimum speed.~(ii) It calculates time-optimal transitions for transitions that appeared at~(i).~(iii) It preform~\astareps-like search to find sum-time-optimal path from~$s_{\text{start}}$ to~$s_{\text{goal}}$ with significantly less running time compare to an optimal path.  At each iteration, the algorithm uses a \textsc{Focal} list to decide which node to expand. In addition, we denote~$E_{\text{opt}}$ as the set of time-optimal edges in the graph and~$e_n$ as the edge of node~$n$ which start at~$n.\text{parent}$ and end at~$n.\text{configuration}$.

% \begin{equation}
%     \textsc{Focal} = \left\{ \text{n} \in \textsc{Open} \mid f(n) \leq \varepsilon \underset{n'\in \textsc{Open}}{\min} f(n') \right\}
%     \label{eq:focal}
% \end{equation}

% % \begin{algorithm}[H]
% % \SetAlgoLined
% % \caption{\tstareps}
% % \BlankLine
% % %\KwIn{map,~$\mathbf{s}_\text{start}$,~$\mathbf{s}_\text{goal}$, \varepsilon, wind}
% % \KwIn{$\text{map}, \mathbf{s}_\text{start}, \mathbf{s}_\text{goal}, \varepsilon, \text{wind}$}
% % \KwOut{sub-optimal minimum-time path from~$\mathbf{s}_\text{start}$ to~$\mathbf{s}_\text{goal}$}
% % \BlankLine
% % Find the shortest path by using minimum speed Dubins paths\\
% % Calculate time-optimal transitions for transitions that appeared at 1\\
% %~\astareps-like search\\
% % \end{algorithm}
% % \newpage

% \begin{algorithm}
% % Add meaning to input variables
% \caption{\text{\astareps-like search}}
% \KwIn{$\text{map}, \mathbf{s}_\text{start}, \mathbf{s}_\text{goal}, \varepsilon, \text{wind}$}
% \KwOut{$\text{sub-optimal minimum-time path from} \mathbf{s}_\text{start} \text{to} \mathbf{s}_\text{goal}$}
% % Ask Oren to use path or trajectory.
% \BlankLine
% \While{$\textsc{Open} \neq \emptyset$}{
%    ~$\text{Next\_to\_expand} \leftarrow \texttt{Find\_next\_node(\textsc{Open})}$\\
%    ~$\textsc{Open} \leftarrow \textsc{Open} \setminus\text{Next\_to\_expand}$\\
%    ~$\textsc{Closed} \leftarrow \textsc{Closed} \cup \text{Next\_to\_expand}$\\
%     \For{$\text{s} \in \text{succ(Next\_to\_expand.configuration)}$}{
%        ~$\text{cost\_from\_parent} \leftarrow \texttt{cost(s,Next\_to\_expand.configuration)}$\\
%        ~$\text{s.f} = \text{Next\_to\_expand.g} + \text{cost\_from\_parent} + \text{h(s)}$\\
%         \If{$\text{s} \in \text{OPEN or s} \in \textsc{Closed}$}
%         {
%             \text{Check if s the current path to s is better than the one already found and update \textsc{Open} and \textsc{Closed}}
%         }
%     }
% }
% \label{astareps-like}
% \end{algorithm}


% \begin{algorithm}[H]
%   \DontPrintSemicolon
%   \SetKwFunction{FMain}{\text{Find\_next\_node}}
%   \SetKwProg{Fn}{Function}{:}{}
%   \Fn{\FMain{\textsc{Open}}}{
%     \uIf{$\exists\, n \in \textsc{Focal} \land e_n \in E_{\text{opt}}$}{
%              \KwRet~$\underset{n \in \textsc{Focal} \land e_n \in E_{\text{opt}}}{\argmin} f(n)$\;}
% 	 \Else{
% 	    calculate time-optimal transition for \text{OPEN.top() }\;
% 	    \KwRet~$\text{Next} \leftarrow \texttt{Find\_next\_node}(\textsc{Open})$}
% }
% \label{find_next}
% \end{algorithm}


% \begin{algorithm}[H]
%   \DontPrintSemicolon
%   \SetKwFunction{FMain}{cost}
%   \SetKwProg{Fn}{Function}{:}{}
%   \Fn{\FMain{successor, parent}}{
%     \uIf{$e(parent, configuration) \in E_{\text{opt}}$}{
% 	         \KwRet time-optimal cost from parent to successor\;}
% 	 \Else{
% 	    \KwRet lower bound from parent to successor\;}
% }
% \label{cost_func}
% \end{algorithm}


% - appendix.tex --------------------------------------------------------------

% \adjustbox{margin=1em,width=\textwidth,set height=4cm,set depth=4cm,frame,center}{\includegraphics[scale=0.6]{pics/Lower bound quality}}
% {\includegraphics[scale=0.6]{pics/Lower bound quality}}
%The colored area around each line represents the range of 60\% of the lower bounds estimation for the true cost.

%This corresponds to the constraint that the wind magnitude is smaller than the minimum speed of the vehicle~$v_{\textup{min}}$, i.e., 


% The lower bound that uses ground speed is better than the version that assumes the vehicle can travel at maximum speed and turn with the smallest radius.
%For any wind force, the lower bound that incorporates ground speed provides a better estimate of the true cost.

\ignore{
%that is not known beforehand, so the time-optimal paths need to be computed on the fly. Then,
{\color{brown}
The proposed \tstareps{} algorithm utilizes lower bounds for true cost of the path to reduce the number of computed of computed time-optimal paths, and thus reduce also the overall computational time.
This is crucial for dynamic environments because the true cost depends on the specific location and cannot be precomputed as for static environment.
Therefore, the appendix provides more detail description of the utilized lower bounds in the proposed algorithm.

This work consider a case with a  constant wind~$\vec{w} = (w_x, w_y)$ that is not known beforehand, so the time-optimal paths need to be computed on the fly. Then, the model~(\ref{eq:dynamics}) of the vehicle changes to
\begin{equation}
\left(\begin{matrix}
    \dot{x}(t)\\
    \dot{y}(t)\\
    \dot{\theta}(t)
\end{matrix} \right)
=
\left(\begin{matrix}
    v(t) \cos\theta(t) + w_x\\
    v(t) \sin\theta(t) + w_y\\
    u(t)
\end{matrix} \right).
\end{equation}

To simplify the model, it is assumed that the vehicle is allowed only when the wind magnitude is less than the minimum speed of the vehicle~$v_{\textup{min}}$, i.e., the vehicle goes forward
\begin{equation}
    \vert \vec{w} \vert < v_{\textup{min}}.
    \label{eq:windlimit}
\end{equation}


The wind also significantly influences turning capabilities of the vehicle (in the reference frame of the ground). 
The smallest turn radius can be achieved when flying directly against the wind and it is further denoted as the lower bound radius~$\rho_\text{LB}$ 
    \begin{equation}
        \rho_\text{LB} = \left(1-\frac{\vert \vec{w} \vert}{v_{\textup{min}}}\right) \, \rho _{\min}.
        \label{r_min_wind}
    \end{equation}
% \DP{This lower bound radius is also used in the heuristic function~$h$ of the algorithm in windy conditions.
% In those conditions, the estimation of the cost to reach the goal from node~$n$,~$h(n)$, is the length of Dubins path using~$\rho_{\min}$ divided by the vehicle's maximum speed add to the wind magnitude~$v_{\max} + \vert \vec{w} \vert$}.

Then, a lower bound estimate of true length of path between two configurations~$s_1$ and~$s_2$ can be determined based on length~$\mathcal{L}(s_1, s_2, \rho_\text{LB})$ of Dubins path with the lower bound radius.
Further, if the lower bond length is divided by upper bound speed (in the reference frame of the ground) it provides a lower bound on the true cost (travel time).

In this paper, we provide two lower bound based on how the upper bound speed is determined.
First lower bound~$\text{LB}_1$ computed the maximum speed as a sum of maximum speed and wind magnitude
\begin{equation}
    \text{LB}_1(s_1, s_2) = \frac{\mathcal{L}(s_1, s_2, \rho_\text{LB})}{v _{\max} + \vert \vec{w} \vert}.
    \label{LB1}
\end{equation}

The second lower bound~$\text{LB}_2$ reflect the direction between end configurations by computing the ground speed~$\vec{v_{\textup{G}}}$ in the given direction~$\vec{d}$.
The direction is determined based on end configuration~$s_1$ and~$s_2$ as
\begin{equation}
    \vec{d} = \frac{s_{2}^\text{xy} - s_{1}^\text{xy}}{\vert s_{2}^\text{xy} - s_{1}^\text{xy} \vert},
\end{equation}
where~$s_{i}^\text{xy}$ stands for~$x,y$ coordinates of configuration~$s_i$.

The ground speed~$\vec{v_{\textup{G}}}$ vector can be expressed by the airspeed~$\vec{v}$ and wind~$\vec{w}$
\begin{equation}
\vec{v_{\textup{G}}} = \vec{v} + \vec{w}.
\end{equation}

Because (\ref{eq:windlimit}) holds, the maximum ground speed occurs at maximum airspeed of vehicle, i.e.,~$\vert \vec{v} \vert = v_\text{max}$.
The angle between~$\vec{v_{\textup{G}}}$ and~$\vec{w}$ can be written as
\begin{equation}
    \cos \angle (\vec{v_{\textup{G}}}, \vec{w}) = \frac{\vec{d} \cdot \vec{w}}{\vert \vec{w} \vert}.
\end{equation}

Then, the ground speed can be expressed based cosine rule as
\begin{equation}
    \vert \vec{v_{\textup{G}}} \vert = \vec{d} \cdot \vec{w} + \sqrt{( \vec{d} \cdot \vec{w} )^2 + v _{\max}^2 -\vert \vec{w} \vert ^2 }.
\end{equation}

Finally, the second lower bound~$\text{LB}_2$ is computed as
\begin{equation}
    \text{LB}_2(s_1, s_2) = \frac{\mathcal{L}(s_1, s_2, \rho_\text{LB})}{\vert \vec{v_{\textup{G}}} \vert }.
    \label{LB2}
\end{equation}

     
Fig.~\ref{fig:lower_bound_wind} shows the average ratio between the lower bound and the true cost vs. wind force. 
For both lower bounds, their estimation of the true cost becomes worse with increasing wind force.
Notice that~$\text{LB}_2$ is more informative than~$\text{LB}_1$ because the direction enables reducing the upper bound on the ground speed. 
% The lower bound that uses ground speed is better than the version that assumes the vehicle can travel at maximum speed and turn with the smallest radius.
%For any wind force, the lower bound that incorporates ground speed provides a better estimate of the true cost.
In static environmental conditions, both lower bounds reduce to vehicle's minimum speed Dubins path divided by its maximum speed.

}

\ignore{
Moreover, it considers that the vehicle can not travel backward.

\item \textit{System dynamic model} \\
    To ensure that, the wind force needs to be less than its minimum speed:
    \begin{equation}
        \vert \vec{w} \vert < v_{\textup{min}}.
    \end{equation}
    Where~$\vec{w}=(w_x, w_y)$ is a wind vector.
    
    Let add~$\vec{w}$ to the dynamic model of the robotic-system as follow:
    \begin{equation}
        \begin{cases}
        \dot{x}(t) = v(t) \cos\theta(t) + w_x, \\
        \dot{y}(t) = v(t) \sin\theta(t) + w_y, \\
        \dot{\theta}(t) = u(t).
        \end{cases}
    \end{equation}
    
\subsection{Lower bound for true cost}
    Regarding dynamic environmental conditions, two lower bound options for the algorithm were examined.
    The lower bound for the turning radius is determined based on the wind speed. 
    Let assume, w.l.o.g, that the wind direction is parallel to the x-axis, and thus~$w_y= 0$. 
    Then the wind can be easily described by its relative speed to the minimum airspeed of the vehicle~$v_{\min}$
    \begin{equation}
    w_x = \alpha\, v_{\min} ,  \: \: 0 \leq \alpha < 1.
    \end{equation}

    The lower bound radius~(in the reference frame of the ground) is determined based on the minimum turning radius~$\rho _{\min}$
    \begin{equation}
        \rho_\text{LB} = (1-\alpha) \, \rho _{\min}.
        \label{r_min_wind}
    \end{equation}
    This radius is the actual minimum turning radius in this wind conditions. 
    
        % The first option of the lower bound assumes that the vehicle can travel at maximum-speed and turn with the minimum turning radius between consecutive configurations:
    The first option of the lower bound is the same as in static conditions but considers the wind. 
    \begin{equation}
        \text{LB}_1 = \frac{\text{\emph{Dubins path}}(\rho_\text{LB})}{v _{\max} + \vert \vec{w} \vert}.
        \label{LB1}
    \end{equation}
    Where \text{\emph{Dubins path}}($\rho$) denotes the Dubins path using turning radius~$\rho$.
    
    The second option of lower bound is to use the ground speed,~$v_{\textup{ground}}$, which is based on the direction of the transition between the consecutive configurations:
    \begin{equation}
        s_{i_\text{position}} = s_i (\hat{x} + \hat{y})^T.
    \end{equation}
    
    \begin{equation}
        \hat{s} = \frac{s_{2_\text{position}} - s_{1_\text{position}}}{\vert s_{2_\text{position}} - s_{1_\text{position}} \vert}.
    \end{equation}
    
    \begin{equation}
        v_{\textup{ground}} = \hat{s} \cdot \vec{w} + \sqrt{(\hat{s} \cdot \vec{w})^2 + v _{\max}^2 -\vert \vec{w} \vert ^2 }.
    \end{equation}
    
    \begin{equation}
        \text{LB}_2 = \frac{\text{\emph{Dubins path}}(\rho_\text{LB})}{v_{\textup{ground}}}.
        \label{LB2}
    \end{equation}
    
     Where~$s_{i_\text{position}}$ refers to the~$x$ and~$y$ coordinates of configuration~$s_i$. 
     As shown in the lower bound analysis in static conditions, both lower bounds do not consider obstacles.
     
    %  Fig.~\ref{fig:lower_bound_wind} shows a comparison between both lower bound for the time-optimal transitions when higher is better since it leads to tighter lower bound and to better estimation of the actual cost of the time-optimal transition. 
    %  As can be seen, the lower bound that uses ground speed is better than the version that assumes the vehicle can travel at maximum speed and turn with the smallest radius.
    Fig.~\ref{fig:lower_bound_wind} shows the average ratio between the lower bound and the true cost vs. wind force. 
    For both lower bounds, their estimation of the true cost becomes worse with increasing wind force.
    % The lower bound that uses ground speed is better than the version that assumes the vehicle can travel at maximum speed and turn with the smallest radius.
    For any wind force, the lower bound that incorporates ground speed provides a better estimate of the true cost.
    In static environmental conditions, both lower bounds reduce to vehicle's minimum speed Dubins path divided by its maximum speed.
}

    

    
\ignore{

\subsection{Computation of time optimal transitions}
    The library done by~\cite{Wolek} was modified to compute time-optimal transitions with consideration of wind. \footnote{\url{https://github.com/CRL-Technion/Variable-speed-Dubins-with-wind}}

}

% \begin{enumerate}[A.]
    
%     \item \textit{Lower bound for true cost} \\
%     Regarding dynamic environmental conditions, two lower bound options for the algorithm were examined.
%     The lower bound for the turning radius is determined based on the wind speed. 
%     Let assume, w.l.o.g, that the wind direction is parallel to the x-axis, and thus~$w_y= 0$. 
%     Then the wind can be easily described by its relative speed to the minimum airspeed of the vehicle~$v_{\min}$
%     \begin{equation}
%     w_x = \alpha\, v_{\min} ,  \: \: 0 \leq \alpha < 1.
%     \end{equation}
    
%     The lower bound radius~(in the reference frame of the ground) is determined based on the minimum turning radius~$\rho _{\min}$
%     \begin{equation}
%         \rho_\text{LB} = (1-\alpha) \, \rho _{\min}.
%         \label{r_min_wind}
%     \end{equation}
%     This radius is the actual minimum turning radius in this wind conditions. 
    
%     % The first option of the lower bound assumes that the vehicle can travel at maximum-speed and turn with the minimum turning radius between consecutive configurations:
%     The first option of the lower bound is the same as in static conditions but considers the wind. 
%     \begin{equation}
%         \text{LB}_1 = \frac{\text{\emph{Dubins path}}(\rho_\text{LB})}{v _{\max} + \vert \vec{w} \vert}.
%         \label{LB1}
%     \end{equation}
%     Where \text{\emph{Dubins path}}($\rho$) denotes the Dubins path using turning radius~$\rho$.
    
%     The second option of lower bound is to use the ground speed,~$v_{\textup{ground}}$, which is based on the direction of the transition between the consecutive configurations:
%     \begin{equation}
%         s_{i_\text{position}} = s_i (\hat{x} + \hat{y})^T.
%     \end{equation}
    
%     \begin{equation}
%         \hat{s} = \frac{s_{2_\text{position}} - s_{1_\text{position}}}{\vert s_{2_\text{position}} - s_{1_\text{position}} \vert}.
%     \end{equation}
    
%     \begin{equation}
%         v_{\textup{ground}} = \hat{s} \cdot \vec{w} + \sqrt{(\hat{s} \cdot \vec{w})^2 + v _{\max}^2 -\vert \vec{w} \vert ^2 }.
%     \end{equation}
    
%     \begin{equation}
%         \text{LB}_2 = \frac{\text{\emph{Dubins path}}(\rho_\text{LB})}{v_{\textup{ground}}}.
%         \label{LB2}
%     \end{equation}
    
%      Where~$s_{i_\text{position}}$ refers to the~$x$ and~$y$ coordinates of configuration~$s_i$. 
%      As shown in the lower bound analysis in static conditions, both lower bounds do not consider obstacles.
     
%     %  Fig.~\ref{fig:lower_bound_wind} shows a comparison between both lower bound for the time-optimal transitions when higher is better since it leads to tighter lower bound and to better estimation of the actual cost of the time-optimal transition. 
%     %  As can be seen, the lower bound that uses ground speed is better than the version that assumes the vehicle can travel at maximum speed and turn with the smallest radius.
%     Fig.~\ref{fig:lower_bound_wind} shows the average ratio between the lower bound and the true cost vs. wind force. 
%     For both lower bounds, their estimation of the true cost becomes worse with increasing wind force.
%     % The lower bound that uses ground speed is better than the version that assumes the vehicle can travel at maximum speed and turn with the smallest radius.
%     For any wind force, the lower bound that incorporates ground speed provides a better estimate of the true cost.
%     In static environmental conditions, both lower bounds reduce to vehicle's minimum speed Dubins path divided by its maximum speed.
%     \item \textit{Computation of time optimal transitions} \\
%     The library done by~\cite{Wolek} updated to compute time-optimal transitions with consideration of wind. \footnote{\url{https://github.com/CRL-Technion/Variable-speed-Dubins-with-wind}}
% \end{enumerate}

\begin{figure}[!t]
    \centering
    % \adjustbox{margin=1em,width=\textwidth,set height=4cm,set depth=4cm,frame,center}{\includegraphics[scale=0.6]{pics/Lower bound quality}}
    \includesvg[scale=0.5]{pics/Lower bound quality for paper with fill of 60 percent.svg}
    % {\includegraphics[scale=0.6]{pics/Lower bound quality}}
    \caption{The average ratio between the lower bound and time-optimal costs vs. wind's modulus~(solid lines). 
    %The colored area around each line represents the range of 60\% of the lower bounds estimation for the true cost.
    {\color{brown}The colored area around each line represents 60\% non-parametric confidence interval of the true value.}
    }
    \label{fig:lower_bound_wind}
\end{figure}
}


